FWD: Real-time Novel View Synthesis with Forward Warping and Depth

Novel view synthesis (NVS) is a challenging task requiring systems to generate photorealistic images of scenes from new viewpoints, where both quality and speed are important for applications. Previous image-based rendering (IBR) methods are fast, but have poor quality when input views are sparse. Recent Neural Radiance Fields (NeRF) and generalizable variants give impressive results but are not real-time. In our paper, we propose a generalizable NVS method with sparse inputs, called FWD, which gives high-quality synthesis in real-time. With explicit depth and differentiable rendering, it achieves competitive results to the SOTA methods with 130-1000x speedup and better perceptual quality. If available, we can seamlessly integrate sensor depth during either training or inference to improve image quality while retaining real-time speed. With the growing prevalence of depths sensors, we hope that methods making use of depth will become increasingly useful.

==> figures/ablation_figure.tex <==
\begin{figure*}
    \centering
    \begin{tabular}{@{}c@{\hspace{0.5mm}}c@{\hspace{0.5mm}}c@{\hspace{0.25mm} \unskip \vrule \hspace{0.25mm}}c@{\hspace{0.5mm}}c@{\hspace{0.5 mm}}c@{\hspace{0.5mm}}c@{\hspace{0.25mm}\vrule \hspace{0.25mm}}c@{}}
    \multicolumn{3}{c}{\small Input views} & \multicolumn{1}{c}{\small PixelNeRF} & \multicolumn{1}{c}{\small IBRNet} & \multicolumn{1}{c}{\small Ours} & \multicolumn{1}{c}{\small Ours + Depth} & \multicolumn{1}{c}{\small Target Views}\\
    % Input views1 &Input views2 &Input views3 & Novel views 1 &Novel views 2 &Novel views 3\\
    % \text{Input View1} &
    % \text
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}\\
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}&
    \includegraphics[width=0.12\textwidth]{./figures/materials/placeholder.png}\\

    \end{tabular}
    \caption{We compare the qualitative difference for ablation.}
    \label{fig:ablation}
    \vspace{-2mm}
    \end{figure*}

==> figures/system.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.49\textwidth]{figures/costvolumeUnet.pdf}
    \caption{ \textbf{The depth Network $d$.}
    We utilize a cost volume at the bottleneck of UNet to fuse information from multi-views.
    \Ang{Re-draw, Ugly now.}}
\end{figure}

==> figures/teaser_figure_old.tex <==
\begin{figure*}[t!]
	\centering
			{\includegraphics[width=\textwidth]{figures/teaser.pdf}}
    \captionof{figure}{{\bf Efficient View Synthesis from Sparse Views.} We present a method to synthesize images from few input views up to 500$\times$ faster than competing methods. By using an explicit geometric representation, our method can utilize ground truth depth (top), but is robust if it is not available (bottom).
}
	\label{fig:teaser}
\end{figure*}

==> sections/abstract_v2.tex <==
\begin{abstract}
    Novel view synthesis~(NVS) is a challenging task requiring systems to generate photorealistic images of scenes from new viewpoints.
    Conventional image-based rendering~(IBR) represents scenes explicitly, which requires dense image collections and is fundamentally limited by the quality of estimated geometry.
    Recently, Neural Radiance Fields (NeRF) and their generalizable variants have emerged as elegant and effective methods for view synthesis.
    Despite impressive results, they suffer from severe computational bottlenecks, leading to extremely slow speeds.
    In this paper, we propose a \emph{fast} and \emph{generallizable} novel view synthesis method with very \emph{sparse} inputs.
    With explicit depth estimations and differentiable rendering, the proposed method achieves competitive synthesis quality with SOTA methods with orders of magnitude (over 200 $\times$)accelerations. 
\end{abstract}
  


==> sections/experiment_v2.tex <==
\section{Experiments}

The core motivation of our paper is the trade-off between speed and performance for novel view-synthesis:
compared with the current NeRF-style work, we can achieve comparable performance with orders-of-magnitude speedup by explicitly using depths and forward warping,
and obtain superior performance with observed depths, which can be easily collected by concurrent devices.

To this end, the goal of our experiments is to identify the speed and accuracy at which our method can synthesize novel images given sparse inputs. 
We do this by evaluating our methods using standard dataset and metrics, and comparing to the state-of-the-art methods and alternative approaches.
Experiments take place on real data with held-out test scenes and no per-scene optimization.
We additionally conduct ablation experiments to validate the effectiveness of our design. 

\subsection{DTU MVS Benchmark}\label{sec:exp_dtu}

Following PixelNeRF \cite{yu2020pixelnerf}, we use DTU MVS~\cite{jensen2014large} as our primary dataset for evaluation. 
DTU MVS dataset is a real scene dataset consisting of 103 scenes, where a scene contains one or multiple objects placed on a table. 
Images and incomplete depths are collected by the camera and structured light scanner mounted on an industrial robot arm, while corresponding camera poses are provided.
For simplicity, we refer the collected incomplete depths as the ground truth depths.
DTU dataset does not contain humans or personally identifiable information, and scenes are of household objects on tables, which appear unlikely to be offensive.

As stated in ~\cite{yu2020pixelnerf}, this is a challenging dataset since it consists of complex real scenes without clear semantic similarities across scenes.
In addition, images are taken under varying lighting conditions with distinct color inconsistencies between different views.
Further, there are large portions of black background pixels in images, which pose significant challenges to depth estimation and optimizations.
Moreover, with under 100 scenes are available for training, it is prone to overfitting in the training set. 

For fair comparison, we follow the exact same pipelines as PixelNeRF \cite{yu2020pixelnerf} for training and evaluations. 
We employ the same data splitting with 88 training scenes and 15 test scenes, in which there are no shared or highly similar scenes between the two sets.
Images are down-sampled to a resolution of 300 $\times$ 400.
During training, we randomly sample 3 views as input while keeping the rest as target views.
In inference, we choose a set of fixed informative input views shared across all instances.

\input{tables/dtu.tex}
% \input{tables/time_table.tex}

\input{figures/DTU_gt_depth_results.tex}

For evaluation, we calculate the \emph{SSIM}, \emph{PSNR} and learned perceptual image patch similarity~(\emph{LPIPS}) as measurements of synthesis quality.
We additionally count the inference time as another metric: we measure the total inference time of all views on a per-scene basis. 
For DTU, with 3 input views, each scene has 46 inference images.
Inference time is measured on single RTX 2080 Ti GPU.

Because of the GPU memory limitation, for efficient training, we down-sample the input images to 150$\times$200 at the inner model and output at the original resolution 300$\times$400 by adding intermediate upsampling layer in refinement model.
For fair comparison, we measure the inference time of models with 1) low resolution: input and output at 150$\times$200; 2) high resolution: input and output at 300 $\times$ 400; 3) Hybrid: input at 150 $\times$ 200 and output at 300$\times$ 400.

% \subsubsection{Baselines}
\input{tables/method_depth_table.tex}

\noindent\textbf{Baselines.}
We present two main versions of our model: using ground-truth depth (GT), and estimated depth from input views by MVS algorithm (MVS).
The former captures depth via structured light and contains missing regions;
the latter uses pre-trained PatchMatchNet~\cite{wang2019wide} to estimate depth.
Though generalized very well on other dataset without retraining, PatchMatchNet is trained on DTU training dataset,
 so we state depth is available for fairness.
% Since \cite{wang2019wide} uses DTU depth maps during training, this model uses sensor depth during training but not inference.
% Depth is captured using a structured light scanner, and contains many missing regions.
%We use PatchmatchNet to obtain MVS depth, which is a lightweight network based on patch matching which is trained on DTU.
%We therefore consider our model utilizing MVS to have access to depth during training, but not inference.
%Our baseline model does not require ground-truth depth at inference, taking estimations from the pre-trained PatchmatchNet as inputs for the depth network. 
%PatchmatchNet is light-weight depth estimation network based on MVS patch matching which is trained on DTU.
We filter low-confidence depth from the network input.
% We apply filtering to remove low-confidence estimations from our network input.
For each input view, we estimate its depth by taking the other two views are source views.
Note that this setting is very \emph{different} from MVS depth estimation setting and estimations are \emph{inaccurate}, since
(1) the number of source views are far fewer than MVS tasks;
(2) the source views are not selected for optimal estimation.

% These two lines should go somewhere else
%In baseline, we evaluate the robustness of model to inaccurate depth estimations.
%We freeze PatchmatchNet during the training for efficiency.

We compare with PixelNeRF and IBRNet, which are both generalized NeRF and the state-of-the-art.
We use the pre-trained PixelNeRF model and carefully retrain the IBRNet on DTU MVS dataset with the same 3-input-view settings.
Finally, we present two other uses of depth in our model. First, Supervised Depth, which directly regresses sensor depths during training.
Second, Unsupervised Depth, which learns depth only implicitly through end-to-end training.
All baselines and versions of our model are detailed in Table~\ref{tab:method_settings_table}.
%Details of all baselines and versions of our model can be found %in Table~\ref{tab:method_settings_table}.
%PatchmatchNet is trained upon DTU, so we consider our model using MVS Depth to have 

%Even though generalized very well in other datasets without retraining, 
%original PatchmatchNet is trained on DTU MVS training dataset. 
%To this end, for fairness, we claim Ours (MVS Depth) gets access to ground truth depth in Table~\ref{tab:method_settings_table} while we don't provide GT depth directly to model .

% (2) we don't conduct view selection to get optimal view points for depth estimations. 


%We also evaluate the model with extra depth information, captured by structured light scanner.
%The captured depths contain many unavailable regions limited by device capacity.  
%Similar to baseline model, we take the incomplete depth and input images as inputs for depth network.




% \subsubsection{Results.}
\noindent\textbf{Results.}
We show the qualitative results of our model in Figure~\ref{fig:dtu_gt_depth}.
Our model could synthesize high-quality and geometrically correct novel views 
with a 38 FPS~(1.2 seconds for 46 views) speed under large viewpoint changes.
The refinement model faithfully inpaints invisible regions;
also synthesized images have reasonable shadows, light reflection and varying apperance across diffeerneet views.
% Our model could faithfully inpaint invisible regions, generate shadows and varying apperance across views.
% Our method is \Ang{number} $\times$ faster than PixelNeRF and $\times$ faster than IBRNet.


\input{tables/time_table_v2.tex}
\textbf{Quantitative Results.}
% In Table~\ref{tab:dtu}, we evaluate the PSNR, SSIM and LPIPS as 
We report the quantitatively results in Table~\ref{tab:dtu} and inference time in Table~\ref{tab:time}.
Our baseline model achieves comparable performance as PixelNeRF and IBRNet~(lower PSNR while better LPIPS), with about 1300 $\times$ and 141 $\times$ accelerations respectively. 
The results demonstrate that our model could give robust synthesis with inaccurate depth estimations.
With ground truth depths, our model outperforms the existing methods by a large margin for all metrics.


\textbf{Inference Time.}
Due to GPU memory limitations, our model operates at a \emph{hybrid} resolution:
the input images are downsampled to $150\times200$, but we produce $300\times400$-pixel outputs by inserting an upsampling layer in the Refinement module.
Our model thus generates images at the same resolution as the baselines, but this internal downsampling improves our speed and memory footprint.
For fair comparision, we also report the speed of our model without down/upsampling at both high and low resolution.
Table~\ref{tab:time} shows that our model is orders of magnitude faster than the baselines.

%Because of the GPU memory limitation, for efficient training, we down-sample the input images to 150x200 at the inner model and output at the original resolution 300x400 by adding upsampling layer in Refinement model.
%Although all methods output at the same resolution, we provide the inference time without downsampling for fair comparison:
%without downsampling, \emph{FWD + Depth} uses 3.7 second for all novel views while \emph{Ours} uses 4.5 seconds,
%which demonstrates orders-of-magnitude accelerations for current method.
%We report the inference time and corresponding FPS under different resolutions in Table~\ref{tab:time}.
%For efficient training, evaluated is under hybrid which down-samples the input images internally while outputs at the high resolution.
%Our method achieves orders-of-magnitude accelerations for existing method in all resolutions.
% Because of the GPU memory limitation, for efficient training, we down-sample the input images to 150x200 at the inner model and output at the original resolution 300x400 by adding upsampling layer in Refinement model.
% Although all methods output at the same resolution, we provide the inference time without downsampling for fair comparison:
% without downsampling, \emph{FWD + Depth} uses 3.7 second for all novel views while \emph{Ours} uses 4.5 seconds,
% which demonstrates orders-of-magnitude accelerations for current method.

\input{figures/DTU_results_comparison.tex}
\textbf{Qualitative Comparison. }
We show the qualitative comparison between different methods in Figure~\ref{fig:dtu_results_compar}.
All methods demonstrate good ability to inpaint invisible regions.
Our model with ground truth depths achieves visually superior performance compared with the other three methods,
and the results of PixelNeRF and IBRNet tend to be blur objects due to uncertainty. %since they are trained with MSE loss. 
Using explicit 3D representations, our model maintains good geometric consistences across different views,
while the results of PixelNeRF and IBRNet suffer from severe distortions at some view points.
Despite the overall high quality, the model without ground truth depths suffers from inaccurate depth estimations, like the curve of the building (row 1) and hand of Elf.
% Even without ground truth depths, our model could synthesize fine details if depths are easily estimated,
% but also suffer 


\subsection{Ablations}

We evaluate the effectiveness of our designs and study depth in more detail through ablation experiments. 
Our focus is on fast novel view synthesis, so we assess both cost and performance.
%First, we ablate view dependence and transformer fusion. 
%Second, we consider several methods of obtaining depth and their impact on performance in addition to speed.

\input{tables/arch_ablation.tex}
\input{tables/depth_ablation_v2.tex}
\input{figures/depth_figure.tex}

% \emph{Model without transformer.}
% Rather than utilizing a transformer to fuse projected features from different input views, 
% we directly aggregate point clouds obtained from each input view into a complete point cloud and project it to the target view.
% The same refinement module is still utilized.

% \emph{Model without view dependence.}
% We directly project the features into target view.

% In the ablation Table~\ref{tab:design_ablation}, we show that.

% \subsubsection{Design Ablations}
\noindent\textbf{Design Ablations.}
We conduct ablation study in Table~\ref{tab:design_ablation} to investigate the contribution of key components.
To obviate the influence of depth estimations, we  train each model with GT depth.

\emph{Model without transformer} aggregates point clouds from each input view and projects it to the target view.
This method is more efficient since it only renders once without fusion operations.
It is less robust to inaccurate depth estimations since points with inaccurate depths from one input view will occlude points from other views.

\emph{Model without view dependence} removes the view-dependent feature MLP.
This reduces our model's ability to produce reproduce view-dependent effects. 


% \input{figures/ablation_figure.tex}
% \subsubsection{Depth Ablations}
\noindent\textbf{Depth Ablations.}
As discussed before, our method utilizes forward warping with explicit depths.
Consequently, depth estimations would be one of the major bottlenecks of performance.
In this section, we investigate several different ways to utilize the depths in Table~\ref{tab:depth_ablation}.

FWD (GT) and FWD (MVS) are the same as models in Table~\ref{tab:dtu},
which conduct depth completion for depths collected by devices or calculated from PatchmatchNet.

% The model with \emph{UNet Depth} directly regresses depths for each input view through a UNet, whose input is view image.
%The model with \emph{UNet Depth} employs a UNet to regress the depth for each input view individually, with view image as the only input.
%Similar to single image depth estimation, this model doesn't utilize any geometric constraints across input views.
%And the model with \emph{Supervised Depth} uses the same structure as \emph{UNet Depth} while it has the ground-truth depths as supervision for the UNet regressed depths during the training.
FWD (Sup.) predicts depth via a UNet, supervised with GT during training.
FWD (Unsup.) has the same UNet architecture, but depth predictions are unsupervised and trained end-to-end to minimize the reconstruction loss.
FWD (GT) is the only model to use depth at inference.
% but is trained only through backward-flowing gradients
% from the final reconstruction loss.
% All models have no inference depth information except $\emph{GT Depth}$.

Our results demonstrate that our model could get decent performance by directly regressing depths for each input view image individually.
The tiny improvement with depth supervision indicates that our method could learn descent depth estimations only from 2D supervisions. 
The performance gap between FWD (Unsup.) and FWD (MVS) demonstrates that multi view information could boost the performance of depth estimation and the following view synthesis.
We visualize depths across versions of our method in Figure~\ref{fig:depth}.


\subsection{Source View Density Study.}
\input{tables/multi_inputs.tex}

We investigate how our method works when more input views are available, and also provide results of PixelNeRF and IBRNet for reference.
All models are trained with 3 input views and not retrained for more input views.
Volume rendering is increasingly effective as more views are available, since each additional input provides more intersecting rays from which to sample.
Nevertheless, their compute time increases dramatically as input views increase.
In contrast, the proposed method can still run in real-time even with 9 input views present.
With GT depths, our model already faithfully synthesizes regions visible in input views, 
so it gains little improvements from more views except invisible regions.
The quality of depth estimation from MVS improves with more input views, 
leading to distinct performance boosting with 6 input views and longer inference time as well. 
% Our model with GT depths doesn't benefit much from more views since more
% Our model with MVS depths can learn more accurate depths from more input views, which 
% In addition, performance with partial ground truth depth is competitive with both PixelNeRF and IBRNet.
% \note{this is hypothetical response. may have to edit.}



==> sections/experiment_v3.tex <==
\section{Experiments}


==> sections/experiment_v4.tex <==
\input{tables/name_table.tex}

\section{Experiments}
The goal of our paper is \emph{real-time} and \emph{generalizable} novel view synthesis with \emph{sparse} inputs, which can optionally use sensor depths.
To this end, our experiments aim to identify the speed and quality at which our method can synthesize novel images and explore the advantage of explicit depths.
We evaluate our methods on ShapeNet and DTU  datasets, comparing results with the SOTA methods and alternative approaches.
Experiments take place with held-out test scenes and no per-scene optimization.
We conduct ablation experiments to validate the effectiveness of designs.

% Compared with current NeRF-style methods, our method achieves competitive performance while orders-of-magnitude faster with only RGB images as inputs.
% If sensor depths are further available during inference, our method outperforms both IBR and NeRF-style methods by a large margin. 
% Experiments demonstrate that the proposed method is efficient and effective, significantly improve the speed-quality trade-off for NVS.

\par \noindent {\bf Metrics.}
We use the standard image quality metrics PSNR and SSIM~\cite{wang2004image} for evaluations,
and also report LPIPS~\cite{zhang2018unreasonable} since it reflects the image quality perceived by human. 
In addition, inference speeds are measured, and frames per second~(FPS) is reported as an essential metric.
All evaluations are conducted using the same protocol~(same inputs and outputs), and rendering speed are measured on the same platform~(1 2080Ti GPU with 4 CPU cores).
Visual quality is also evaluated by condu cting user studies. 

\par \noindent {\bf Model Variants.}
% To explore the influence of depths, we evaluate several model variants with  different accessibility to depths for training and inference.
% We predefine these models in Table~\ref{tab:name_table}:
% \FWDds uses a pretrained MVS model while trained by photometric loss, and doesn't have depth during inference. 
% \FWD  takes only RGB images during training and inference, learning depths without depth supervisions or pre-training.
% \FWDrgbd gets access to sensor depths during inference and employ $\mathcal{L}_{s}$ for training;
We evaluate three models with various accessibility to depths for training and inference, and we predefine them in Table~\ref{tab:name_table}.
\FWDds utilizes PatchmatchNet~\cite{wang2020patchmatchnet} as the MVS module for depth estimations in complex scenes.
The PatchmatchNet is initialized from officially pre-trained weights on DTU dataset and updated during end-to-end training with photometric and perceptual loss. 
\FWD learns depth estimations in an {\underline U}nsupervised manner from scratch, sharing the same model and settings as \FWDds while PatchmatchNet is randomly initialized without any pretraining.
\FWDrgbd takes sensor depths as additional inputs during both training and inference.
It doesn't use any MVS module since sensor depths provide abundant geometry cues.

PatchmatchNet is pre-trained following typical MVS settings, which has distinct domain gaps between our settings since our input images share much more distant baselines. 
We show the estimated depths from pre-trained PatchmatchNet in Figure~\ref{fig:depth}, which are inaccurate and relatively incomplete after filtering low-confidence regions. 
\input{tables/shapenet.tex}

\input{figures/shapenet.tex}
\input{figures/DTU_gt_depth_results.tex}

\subsection{ShapeNet Benchmarks}
We first evaluate our approach on the category-agnostic view synthesis task on ShapeNet. 
Following the setting as \cite{yu2020pixelnerf}, we train and evaluate a single model on 13 ShapeNet categories.
Each instance contains 24 fixed views of 64 $\times$ 64 resolution.
During training, one random view is selected as input and the rest are served as target views.
For testing, we synthesize all other views from a fixed informative view.
The model is finetuned  with two random input views for 2-view experiments.
We find that U-Net is sufficient for good results on this synthetic dataset without the MVS module. 

As shown in Table~\ref{tab:shapenet}, for image quality, our method achieves comparable PSNR and SSIM with PixelNeRF~\cite{yu2020pixelnerf} and outperforms other methods significantly.
Also, \FWD achieves the best LPIPS results in all methods, indicating a better perceptual quality.
Besides the high-quality synthesis results,\FWD runs at a speed over 300 FPS, which is above 300 $\times$ faster than PixelNeRF.
Quantitative results show that the proposed method achieves much  better speed-quality tradeoff and demonstrate the effectiveness of design.

We show qualitatively results in Figure~\ref{fig:shapenet}, where \FWD gets noticeably superior results than PixelNeRF.
We study visual quality in Sec~\ref{exp:DTU} thoroughly and analyse its reasons.

\subsection{DTU MVS Benchmarks}
\label{exp:DTU}
We further evaluate models on DTU MVS dataset~\cite{jensen2014large}, which is a real scene dataset consisting of 103 scenes.
Each scene contains one or multiple objects placed on a table, while images and incomplete depths are collected by the camera and structured light scanner mounted on an industrial robot arm.
Corresponding camera poses are provided.

As stated in ~\cite{yu2020pixelnerf}, this dataset is challenging since it consists of complex real scenes without apparent semantic similarities across scenes.
Also, images are taken under varying lighting conditions with distinct color inconsistencies between views.
% Further, large portions of black background pixels in images pose significant challenges to depth estimation and optimizations.
Moreover, with only under 100 scenes available for training, it is prone to overfitting in training. 

We follow the same training and evaluation pipelines as PixelNeRF~\cite{yu2020pixelnerf} for all methods to give a fair comparison. 
The data consists of 88 training scenes and 15 test scenes, in which there are no shared or highly similar scenes between the two sets.
Images are down-sampled to a resolution of 300 $\times$ 400.
During training, three input views are randomly sampled, with the rest as target views.
In inference, we choose three fixed informative input views and synthesize other views of the scene.

\input{figures/DTU_results_comparison.tex}

\par \noindent {\bf Baselines.}
We evaluate a set of representatives of generalizable NeRF and IBR methods in two different scenarios: with RGB or RGB-D available as inputs during inference. 

PixelNeRF~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet} and MVSNeRF~\cite{chen2021mvsnerf} are the state-of-the-art generalizable NeRF variants, taking only RGB as inputs.
We use the official PixelNeRF model trained on DTU MVS dataset and carefully retrain the IBRNet and MVSNeRF with the same 3-input-view settings.
We also evaluate PixelNeRF-DS, which is PixelNeRF~\cite{yu2020pixelnerf} supervised with depths as reported in~\cite{deng2021depth}.
Please note that IBRNet and MVSNeRF use different evaluations in their paper, where IBRNet uses  10 views for synthesis and MVSNeRF selects different input views for each target view.
% We also provide evaluation results in this setting in supp..  

A series of IBR methods are also evaluated. 
Since COLMAP~\cite{schoenberger2016mvs} fails to give reasonable outputs with sparse input images,
methods using COLMAP like FVS~\cite{riegler2020free}, DeepBlending~\cite{DeepBlending2018} cannot estimate scene geometry in this setting. 
For these methods, we use depths captured by sensors as estimated depths, which should give upper-bound performance of these methods.
To better cope with missing regions, we add our refinement model to DeepBlending~\cite{DeepBlending2018} and retrain it on DTU dataset, termed Blending-R.

% We also evaluate baselines like Synpts~\cite{aliev2020neural}, which synthesize novel view images given a colored point cloud.
% The point cloud is constructed from RGB-D images.
% Point cloud encoder and image refinement module is employed. 
% We also compare with SVS~\cite{Riegler2021SVS}, EVS~\cite{choi2019extreme} which are representatives of image-based rendering.
% We also implement PerspectiveNet~\cite{novotny2019perspectivenet}, which utilized RGB-D inputs.


\input{tables/dtu_v2.tex}

\par \noindent {\bf Synthesis Results.}
The synthesis results are shown in Figure~\ref{fig:dtu_gt_depth}, where high-quality and geometrically correct novel views are synthesized in real-time (over 35 FPS) under significant viewpoint changes.
Our refinement model faithfully inpaints invisible regions; also, synthesized images have good shadows, light reflection, and varying appearance across views, showing that the method could model view-dependent effects and shadows effectively.

\par \noindent {\bf Quantitative Results.}
We compare proposed methods with a variety of baselines quantitatively in Table~\ref{tab:dtu}.

\emph{Test with RGB.}
The proposed \FWDds gives optimal speed-quality tradeoff among all methods. For quality, it has the best LPIPS and outperforms all other methods except PixelNeRF-DS for PSNR and SSIM.
For speed,  \FWDds enjoys a real-time speed that is orders-of-magnitude faster than existing methods.
Although it utilizes a pre-trained MVS module, we believe the comparison is reasonable since pre-trained depth models are feasible. 
And even training depths can be easily calculated from dense training images.
PixelNeRF-DS utilizes depths as extra supervision during training and has similar PSNR with \FWDds.

\FWD doesn't use a pre-trained MVS module and has worse results than \FWDds, indicating the importance of depth network initialization.
But it still has an obvious speed advantage and comparable quality to other methods, especially for LPIPS. 
MVSNeRF doesn't give satisfactory results since it is not designed for inputs with large baselines.  

\input{tables/arch_ablation.tex}

\emph{Test with RGB-D.}
With sensor depths as additional inputs, \FWDrgbd outperforms all other methods significantly. 
Its speed is even slightly better than \FWD since it needn't run MVS modules. 
Blending-R~\cite{DeepBlending2018} and FVS~\cite{riegler2020free} suffer a low quality since sensor depths are incomplete and noisy, while our end-to-end method enables the model to refine sensor depths and learn robust features optimized for synthesis quality. 
It is still an open problem for generalizable NeRF variants to use sensor depths to get better quality or speed during inference. 

% \par \noindent {\bf PSNR vs. LPIPS.}
% We notice that the proposed method has better LPIPS and worse PSNR compared with generalizable NeRF variants.
% It is because NeRF renders the value of each pixel independently and is trained by L2 loss alone.
% Our method synthesizes target images using the CNN module and employs content loss which is patch-based. 
% We regard it as another advantage to NeRF variants since our results are expected to be more patch-wisely coherent and perceptually appealing.
% Moreover, imperfect depth estimations may cause tiny misalignments for view synthesis, which is not noticed perceptually but leads to distinct PSNR drops.


\par \noindent {\bf Qualitative Results.}
We show qualitative results in Figure~\ref{fig:dtu_results_compar}.
All methods demonstrate good abilities to inpaint invisible regions and faithfully synthesize views.
Our methods consistently give more visually appealing results than other methods, even for \FWD.
Despite high PSNR, Nerf-variants intend to have jittering and high-frequency artifacts at regions with high uncertainty,
while our method gives more smooth and coherent results.
For instance, both NeRF variants and \FWD have difficulties generating regions between two buildings in the first instance (row 1).
The results from NeRF variants have sharp artifacts and distortions, while our method still gives coherent and appealing results, although the geometry is misaligned.  


Given that LPIPS measures image patches' perceptual similarity,  this observation is consistent with Table~\ref{tab:dtu}, where our methods possess much better LPIPS than other methods.
We take it as an advantage of our method since our design allows the model to generate coherent and visually appealing results. 
For NeRF variants, they are trained to render each pixel independently supervised by photometric loss, leading to high PSNR without considering patch-level quality.
Moreover, PSNR is not friendly to our methods since it is sensible to tiny pixel shiftings.  Depth estimations and rendering would introduce tiny pixel shiftings which are not visually perceptible but degrade PSNR results.

\input{tables/user_study.tex}
\par \noindent {\bf User Study.}
We conduct user studies to faithfully evaluate the synthesis quality by asking users to pick the more realistic one given the target images and synthesized results from methods A and B.
All views in the test sets (690 views in total) are evaluated, and each view is judged by three users. 
It is conducted on HIVE platform and preference is shown in Table~\ref{tab:user_study}.
65.6\% of users believe \FWD results are more realistic than PixelNeRF and 77.8\%  of them prefer \FWD to IBRNet results. 
Besides,  nearly all users prefer \FWDds to \FWD and prefer \FWDrgbd to \FWDds, indicating the effectiveness of introducing sensor depths as inputs.
\subsection{Ablations and Analysis}

We evaluate the effectiveness of our designs and study depth in more detail through ablation experiments. 

\input{tables/depth_ablation_v2.tex}
\input{figures/depth_figure.tex}

\noindent\textbf{Design Ablations.}
We conduct ablation study in Table~\ref{tab:design_ablation} to investigate the contribution of key components.
To obviate the influence of depth, we use \FWDrgbd.

\emph{Model without transformer} aggregates point clouds from each input view and projects it to the target view.
This method is more efficient since it only renders once without fusion operations.
It is less robust to inaccurate depth estimations since points with inaccurate depths from one input view will occlude points from other views.

\emph{Model without view dependence} removes the view-dependent feature MLP.
This reduces our model's ability to produce reproduce view-dependent effects. 

% \emph{Model without Position Encoding} doesn't introduce geometric feature as position encoding when fusing rendered feature maps.
% Our results show that the geometric information of input views is very help for fusion.

\noindent\textbf{Depth Analysis and Ablations.}
% The depth quality is usually the bottleneck of IBR methods.
We visualize the depths involved in our model in Figure~\ref{fig:depth}.
Estimating depth from sparse inputs is challenging, and estimated depths by PatchmatchNet pre-trained on DTU are less accurate because of huge baselines between input images. 
From this perspective, our end-to-end design enables the model to construct point clouds optimized for synthesis quality and learn fusion \& refinement models robust to inaccurate depths.
% \Ang{The depth error results are confusing, need further checking.
% The problem may be: depth and feature cannot be joint learned from scracth at the same time.
% I am trying to train the depth network in unsupervised settings first and then jointly train them.}
The influence of depth components is studied in Table~\ref{tab:dtu}. 
MVS model is a crucial component for depth networks~(row 2), providing depth cues based on multi-view geometry and resolving the scale/shift ambiguity. 
Also, Utilizing U-Net can further improve the synthesis quality~(row 3).

Learning depth estimations unsupervised from scratch is challenging ~(row 4). leading to degraded results and depth errors. 
We hypothesize that fusion \& refinement models may not backward strong enough gradients to train the MVS module since they are robust to inaccurate depths. 
% With RGB-D inputs, \FWDrgbd gives perfect depth estimations and superior synthesis results.
% Our results also demonstrate the effectiveness of the MVS model. 
% Although not designed for it, \FWD works as an unsupervised multi-view stereo pipeline and achieve decent results.
% Sensor depths (b) are incomplete and noisy, and our completion results on them (c) faithfully regress the unknown depths.
% Estimating depths using MVS~(PatchMatchNet) on sparse inputs is challenging, resulting in sparse depths (d)  after filtering out low-confidence estimations and requiring completion (e).
% We also show depth estimations from single image by an end-to-end trained U-Net without MVS depths, with (e) and without (f) depth supervision.



% Our results demonstrate that our model could get decent performance by directly regressing depths for each input view image individually.
% The tiny improvement with depth supervision indicates that our method could learn descent depth estimations only from 2D supervisions. 
% The performance gap between FWD (Unsup.) and FWD (MVS) demonstrates that multi view information could boost the performance of depth estimation and the following view synthesis.
% We visualize depths across versions of our method in Figure~\ref{fig:depth}.
% \input{tables/time_analyse.tex}

% \noindent\textbf{Time  Analysis.}
% We report the time used in each stage for single forward pass, which synthesizes 24 target views. 
% The majority time is spent on refinement module, which uses a conventional style-GAN architecture.
% The time spent on renderer and fusion module demonstrates the effectiveness of these modules.

\subsection{Customer collected RGB-D Image}
To validate the effectiveness of the proposed method in real-world applications, we run the proposed method on a self-collected RGB-D dataset.
This RGB-D dataset is collected by iPhone, which includes x~(not yet) scenes of real-world objects.
RGB-D images are collected from 36 different views for each scene, and depth information is read from iPhone directly.  
We show synthesis results in Figure~, which demonstrates the generalization ability of the proposed method and its significant potentials for real applications.
We are actively collecting more RGB-D images for this dataset and hope it     
will facilitate novel view synthesis and other applications with RGB-D images.




% \subsection{Common Objects in 3D}
% We evaluate our method on Common OBjects in 3D dataset~\cite{reizenstein2021common}, which is a large-scale Real-life 3D category dataset.


% \input{tables/multi_inputs.tex}
% \textbf{Source View Density.}
% We investigate how our method works when more input views are available, and also provide results of PixelNeRF and IBRNet for reference.
% All models are trained with 3 input views and not retrained for more input views.
% Volume rendering is increasingly effective as more views are available, since each additional input provides more intersecting rays from which to sample.
% Nevertheless, their compute time increases dramatically as input views increase.
% In contrast, the proposed method can still run in real-time even with 9 input views present.
% With GT depths, our model already faithfully synthesizes regions visible in input views, 
% so it gains little improvements from more views except invisible regions.
% The quality of depth estimation from MVS improves with more input views, 
% leading to distinct performance boosting with 6 input views and longer inference time as well. 



% \subsection{Customer collected RGB-D Image}
% To demonstrate a potential application of our method, we collect a customer RGB-D dataset with iPhone. 

==> sections/experiment_v5.tex <==
\input{tables/name_table.tex}

\section{Experiments}
The goal of our paper is \emph{real-time} and \emph{generalizable} novel view synthesis with \emph{sparse} inputs, which can optionally use sensor depths.
To this end, our experiments aim to identify the speed and quality at which our method can synthesize novel images and explore the advantage of explicit depths.
We evaluate our methods on ShapeNet~\cite{chang2015shapenet} and DTU~\cite{jensen2014large} datasets, comparing results with the SOTA methods and alternative approaches.
Experiments take place with held-out test scenes and no per-scene optimization.
We conduct ablations to validate the effectiveness of designs.

% Compared with current NeRF-style methods, our method achieves competitive performance while orders-of-magnitude faster with only RGB images as inputs.
% If sensor depths are further available during inference, our method outperforms both IBR and NeRF-style methods by a large margin. 
% Experiments demonstrate that the proposed method is efficient and effective, significantly improve the speed-quality trade-off for NVS.

\par \noindent {\bf Metrics.}
To measure image quality, we report the standard image quality metrics PSNR and SSIM~\cite{wang2004image}.
We also report LPIPS~\cite{zhang2018unreasonable}, and find this metric best reflects the image quality as perceived by humans. 
Visual quality is also evaluated by conducting A/B testing, in which workers select the image most similar to the ground truth from competing methods.
%We fellow a standard A/B paradigm in which workers choose between competing methods the closest to a ground truth image.
%Workers are monitored using a qualifier and sentinel examples, and each test set image is judged by three users.
Inference speeds are measured in frames per second~(FPS).
All evaluations are conducted using the same protocol~(same inputs and outputs), and rendering speed are measured on the same platform~(1 2080Ti GPU with 4 CPU cores).
For full details see supplement.
%Each image is judged by three workers; workers are monitored by 
%All synthesized views in the test set are evaluated, and each view is judged by three users.
%Workers are 
%All views in the test sets (690 views in total) are evaluated, and each view is judged by three users. 
%It is conducted on the HIVE platform, and preference is shown in Table~\ref{tab:user_study}.

\par \noindent {\bf Model Variants.}
We evaluate three models with various accessibility to depths for training and inference, and we predefine them in Table~\ref{tab:name_table}.
\FWDds utilizes PatchmatchNet~\cite{wang2020patchmatchnet} as the MVS module for depth estimations in complex scenes.
The PatchmatchNet is initialized from officially pre-trained weights on DTU dataset and updated during end-to-end training with photometric and perceptual loss. 
\FWD learns depth estimations in an {\underline U}nsupervised manner from scratch, sharing the same model and settings as \FWDds while PatchmatchNet is randomly initialized without any pretraining.
\FWDrgbd takes sensor depths as additional inputs during both training and inference.
It doesn't use any MVS module since sensor depths provide abundant geometry cues.

PatchmatchNet is pre-trained following typical MVS settings, which has distinct domain gaps between our settings since our input images share much more distant baselines. 
We show the estimated depths from pre-trained PatchmatchNet in Figure~\ref{fig:depth}, which are inaccurate and relatively incomplete after filtering low-confidence regions. 

\input{figures/shapenet.tex}
\input{tables/shapenet.tex}

\input{figures/DTU_gt_depth_results.tex}

\subsection{ShapeNet Benchmarks}
We first evaluate our approach on the category-agnostic view synthesis task on ShapeNet. 
Following the setting as \cite{yu2020pixelnerf}, we train and evaluate a single model on 13 ShapeNet categories.
Each instance contains 24 fixed views of 64 $\times$ 64 resolution.
During training, one random view is selected as input and the rest are served as target views.
For testing, we synthesize all other views from a fixed informative view.
The model is finetuned  with two random input views for 2-view experiments.
We find that U-Net is sufficient for good results on this synthetic dataset without the MVS module. 


We show qualitative comparisons to PixelNeRF in Figure~\ref{fig:shapenet}, where \FWD gets noticeably superior results.
Our synthesized results are more realistic and closely matching to target views, while PixelNeRF's results intend to be blurry.
We observe the same trend in the DTU benchmark and evaluate the visual quality quantitatively there.
% \Ang{Chris note: I'm torn on whether we should be consistent with DTU and report qualitative results first. Also, I think we need to describe baselines here, possibly with a bold section. Finally, should Figure 4 be above Table 2? I think the rule is typically figures should be above tables, but not sure since we talk about the table first.}

We show quantitative results in Table~\ref{tab:shapenet}, adding SRN~\cite{NEURIPS2019_b5dc4e5d} and DVR~\cite{DVR} as other baselines. 
Our method outperforms others significantly for LPIPS, indicating a much better perceptual quality,  as corroborated by qualitative results.
PixelNeRF has a slightly better PSNR while its results are blurry. 
Most importantly, \FWD runs at a speed of over 300 FPS, which is 300 $\times$ faster than PixelNeRF.


\subsection{DTU MVS Benchmarks}
\label{exp:DTU}
We further evaluate models on DTU MVS dataset~\cite{jensen2014large}, which is a real scene dataset consisting of 103 scenes.
Each scene contains one or multiple objects placed on a table, while images and incomplete depths are collected by the camera and structured light scanner mounted on an industrial robot arm.
Corresponding camera poses are provided.

As stated in ~\cite{yu2020pixelnerf}, this dataset is challenging since it consists of complex real scenes without apparent semantic similarities across scenes.
Also, images are taken under varying lighting conditions with distinct color inconsistencies between views.
% Further, large portions of black background pixels in images pose significant challenges to depth estimation and optimizations.
Moreover, with only under 100 scenes available for training, it is prone to overfitting in training. 

We follow the same training and evaluation pipelines as PixelNeRF~\cite{yu2020pixelnerf} for all methods to give a fair comparison. 
The data consists of 88 training scenes and 15 test scenes, in which there are no shared or highly similar scenes between the two sets.
Images are down-sampled to a resolution of 300 $\times$ 400.
During training, three input views are randomly sampled, with the rest as target views.
In inference, we choose three fixed informative input views and synthesize other views of the scene.

\input{figures/DTU_results_comparison.tex}
\input{figures/user_study.tex}

\par \noindent {\bf Baselines.}
We evaluate a set of representatives of generalizable NeRF and IBR methods in two different scenarios: with RGB or RGB-D available as inputs during inference. 

PixelNeRF~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet} and MVSNeRF~\cite{chen2021mvsnerf} are the state-of-the-art generalizable NeRF variants, taking only RGB as inputs.
We use the official PixelNeRF model trained on DTU MVS dataset and carefully retrain the IBRNet and MVSNeRF with the same 3-input-view settings.
We also evaluate PixelNeRF-DS, which is PixelNeRF~\cite{yu2020pixelnerf} supervised with depths as reported in~\cite{deng2021depth}.
Please note that IBRNet and MVSNeRF use different evaluations in their paper, where IBRNet uses  10 views for synthesis and MVSNeRF selects different input views for each target view.
% We also provide evaluation results in this setting in supp..  

A series of IBR methods are also evaluated. 
Since COLMAP~\cite{schoenberger2016mvs} fails to give reasonable outputs with sparse input images,
methods using COLMAP like FVS~\cite{riegler2020free}, DeepBlending~\cite{DeepBlending2018} cannot estimate scene geometry in this setting. 
For these methods, we use depths captured by sensors as estimated depths, which should give upper-bound performance of these methods.
To better cope with missing regions, we add our refinement model to DeepBlending~\cite{DeepBlending2018} and retrain it on DTU dataset, termed Blending-R.

% We also evaluate baselines like Synpts~\cite{aliev2020neural}, which synthesize novel view images given a colored point cloud.
% The point cloud is constructed from RGB-D images.
% Point cloud encoder and image refinement module is employed. 
% We also compare with SVS~\cite{Riegler2021SVS}, EVS~\cite{choi2019extreme} which are representatives of image-based rendering.
% We also implement PerspectiveNet~\cite{novotny2019perspectivenet}, which utilized RGB-D inputs.

% \input{tables/user_study.tex}

\par \noindent {\bf Qualitative Results.}
Synthesis results are shown in Figure~\ref{fig:dtu_gt_depth}, where high-quality and geometrically correct novel views are synthesized in real-time (over 35 FPS) under significant viewpoint changes.
Our refinement model faithfully inpaints invisible regions; also, synthesized images have good shadows, light reflection, and varying appearance across views, showing the efficacy of feature-dependent MLP.
With sensor depths, results can be further improved.
% FWD can use depth supervision or depth input if available to improve results.

We show comparisons to baselines in Figure~\ref{fig:dtu_results_compar}. 
FWD provides noticeably better results than baselines across different depth settings.
When sensor depth is not available, baselines IBRNet and PixelNeRF become blurry in areas of high detail such as the buildings in the top row.
While our unsupervised model \FWD gives more realistic and sharper images. 
When depth is available, baseline Blending-R produces more cogent outputs, but still struggles to distinguish objects from the background, such as in the middle row.
In contrast, \FWD produces sharper images without depth, and \FWDrgbd improves detail when depth is available.




%MOVE As indicated by LPIPS number, our methods consistently give more perceptual high-quality results than other methods, even comparing \FWD with PixelNeRF.
% Despite high PSNR, Nerf-variants have distinct jittering and distortions,
% while our method gives more realistic and coherent results.
%For instance, both NeRF variants and \FWD have difficulties generating regions between two buildings in the first instance (row 1).
%The results from NeRF variants have sharp artifacts and distortions, while our method still gives coherent and appealing results, although the geometry is slightly misaligned.  

%Our method gives perceptually better results than others, which is supported by LPIPS numbers and qualitative comparisons. 
%We hypothesize that it is because our model generates novel views based on semantic features, considering both local and global information.
%NeRF variants are trained to render each pixel independently supervised by photometric loss, leading to high PSNR while not considering patch information.
%Moreover, PSNR is sensible to tiny pixel shiftings.
%In our model, depth estimations, geometric transformation, and rendering would introduce misalignments that are not visually perceptible.

\input{tables/dtu_v2.tex}


\par \noindent {\bf Quantitative Results.}
We first evaluate synthesis quality by user study.
We fellow a standard A/B paradigm in which workers choose between competing methods the closest to a ground truth image.
Workers are monitored using a qualifier and sentinel examples.
All views in the test set (690 in total) are evaluated, and each view is judged by three workers. 


User study results are consistent with qualitative observations. In Table~\ref{tab:user_study}, 
we compare FWD to baselines both when depth is available and when depth is available.
In both cases, FWD is chosen by users as more closely matching ground truth images than all baselines the majority of the time.
For instance, \FWD is selected over PixelNeRF in 65.6\% of examples, and 77.8\% compared to IBRNet. 
% \Ang{Chris note: we plan on changing A/B tests to compare to all baselines in a similar manner to the PSNR/LPIPS table. We will probably present this as a bar chart.}
%Besides, nearly all users prefer \FWDds to \FWD and prefer \FWDrgbd to \FWDds, indicating the effectiveness of introducing sensor depths as inputs.

We also compare FWD with baselines using automated view synthesis metrics, along with inference speed, in Table~\ref{tab:dtu}.
We consider three depth availability settings: no depth, depth during training only, and depth during both training and inference.
Across settings, FWD is competitive with baselines across metrics, while having the fastest speed.
Notably, NeRF variants such as PixelNeRF, IBRNet, MVSNeRF, and PixelNeRF-DS are two orders of magnitude slower.
In addition, when depth is available at both train and test time, \FWDrgbd performance is significantly above all alternatives. 

The exception to highly competitive performance across metrics is in the no-depth setting, where \FWD PSNR and SSIM results are weaker than PixelNeRF and IBRNet. 
Nevertheless, without depth \FWD still has better LPIPS, which is more reflective of human judgment, as corroborated by A/B tests in Table~\ref{tab:user_study}.
Figure~\ref{fig:dtu_results_compar} illustrates the disparity between comparisons using PSNR and LPIPS. 
Backward warping methods such as PixelNeRF and IBRNet tend to have aligned but blurred outputs, whereas forward warping methods such as \FWD yield outputs with imperfect alignment but clearer images.
Alignment is more closely measured by PSNR and SSIM, while LPIPS and human judgment prioritize sharp images.

Baseline comparisons also show alternative forward warping methods, which increase speed, do not create images competitive with our method.
For instance, FVS and Blending-R have PSNR at least 5db lower than \FWDrgbd.
In the non-depth setting, SynSin has a PSNR of 1.76 lower than \FWD, along with LPIPS .047 worse.

%The proposed \FWDds gives optimal speed and quality among all methods, with the best perceptual quality~(LPIPS) and second-best PSNR and SSIM.
%\FWDds enjoys a real-time speed, orders-of-magnitude faster than existing methods~(1000$\times$ faster than PixelNeRF).
%Although it utilizes a pre-trained MVS module, we believe the comparison is reasonable since pre-trained depth models are feasible to use. 
%Also, training depths can be easily calculated by MVS algorithms since the training images are dense.
%PixelNeRF-DS trained with extra depth supervision has similar PSNR but worse LPIPS with \FWDds.

% Our unsupervised model \FWD doesn't use a pre-trained MVS module and has worse results than \FWDds, indicating the importance of depth network initialization.
% Although it has worse PSNR than other methods, it gives perceptually high-quality results 
%Our unsupervised model \FWD has a significant speed advantage and competitive quality to other methods:
%although it has a lower PSNR than other methods, it provides perceptually high-quality results since it has the best LPIPS and is noticeably preferred 
%to other methods in user study shown later.
%Meanwhile, it runs above $1000 \times$ faster than PixelNeRF and above $150 \times $ than IBRNet. 
%MVSNeRF doesn't give satisfactory results since it is not designed for inputs with large baselines.  
%We report the results of Synsin~\cite{wiles2020synsin} as a baseline with single input view.


%\emph{Test with RGB-D.}
%With sensor depths as additional inputs, \FWDrgbd outperforms all other methods significantly. 
%Its speed is better than \FWDds since it needn't run MVS modules. 
%Blending-R~\cite{DeepBlending2018} and FVS~\cite{riegler2020free} give worse results since sensor depths are incomplete and noisy, while our end-to-end method enables the model to refine sensor depths and learn robust features optimized for synthesis quality. 
%It is still an open problem for generalizable NeRF variants to use sensor depths to get better quality or speed during inference. 

% \par \noindent {\bf PSNR vs. LPIPS.}
% We notice that the proposed method has better LPIPS and worse PSNR compared with generalizable NeRF variants.
% It is because NeRF renders the value of each pixel independently and is trained by L2 loss alone.
% Our method synthesizes target images using the CNN module and employs content loss which is patch-based. 
% We regard it as another advantage to NeRF variants since our results are expected to be more patch-wisely coherent and perceptually appealing.
% Moreover, imperfect depth estimations may cause tiny misalignments for view synthesis, which is not noticed perceptually but leads to distinct PSNR drops.

\subsection{Ablations and Analysis}

We evaluate the effectiveness of our designs and study depth in more detail through ablation experiments. 
\input{tables/arch_ablation.tex}

\noindent\textbf{Design Ablations.}
We conduct ablation study in Table~\ref{tab:design_ablation} to investigate the contribution of key components.
To obviate the influence of depth, we use \FWDrgbd.

\emph{Model without transformer} aggregates point clouds from each input view and projects it to the target view.
This method is more efficient since it only renders once without fusion operations.
It is less robust to inaccurate depth estimations since points with inaccurate depths from one input view will occlude points from other views.

\emph{Model without view dependence} removes the view-dependent feature MLP.
This reduces our model's ability to produce reproduce view-dependent effects. 

% \emph{Model without Position Encoding} doesn't introduce geometric feature as position encoding when fusing rendered feature maps.
% Our results show that the geometric information of input views is very help for fusion.
\input{figures/desin_ablation_figure.tex}
\noindent\textbf{Depth Analysis and Ablations.}
% The depth quality is usually the bottleneck of IBR methods.
We visualize the depths involved in our model in Figure~\ref{fig:depth}.
Estimating depth from sparse inputs is challenging, and estimated depths by PatchmatchNet pre-trained on DTU are less accurate because of huge baselines between input images. 
From this perspective, our end-to-end design enables the model to construct point clouds optimized for synthesis quality and learn fusion \& refinement models robust to inaccurate depths.
% \Ang{The depth error results are confusing, need further checking.
% The problem may be: depth and feature cannot be joint learned from scracth at the same time.
% I am trying to train the depth network in unsupervised settings first and then jointly train them.}
The influence of depth components is studied in Table~\ref{tab:depth_ablation}. 
MVS model is a crucial component for depth networks~(row 2), providing depth cues based on multi-view geometry and resolving the scale/shift ambiguity. 
Also, Utilizing U-Net can further improve the synthesis quality~(row 3).

Learning depth estimations unsupervised from scratch is challenging ~(row 4). leading to degraded results and depth errors. 
We hypothesize that fusion \& refinement models may not backward strong enough gradients to train the MVS module since they are robust to inaccurate depths. 

\input{figures/depth_figure.tex}
\input{tables/depth_ablation_v2.tex}

% \subsection{Customer collected RGB-D Image}
% To validate the effectiveness of the proposed method in real-world applications, we run the proposed method on a self-collected RGB-D dataset.
% This RGB-D dataset is collected by iPhone, which includes x~(not yet) scenes of real-world objects.
% RGB-D images are collected from 36 different views for each scene, and depth information is read from iPhone directly.  
% We show synthesis results in Figure~, which demonstrates the generalization ability of the proposed method and its significant potentials for real applications.
% We are actively collecting more RGB-D images for this dataset and hope it     
% will facilitate novel view synthesis and other applications with RGB-D images.








==> sections/intro_backup.tex <==
\section{Introduction}

% Given a set of posed images of a scene, novel view synthesis produces photo-realistic images at novel viewpoints.
% Early work on novel view synthesis utilized image-based rendering~(IBR), which generally warps source views to target viewpoints and requires very dense input views to get high-quality synthesis.
% Recently, fast progress has been seen due to advances in differentiable neural rendering and neural scene representations.
% Notably, the recent neural radiance fields (NeRF~\cite{mildenhall2020nerf}) use MLPs to represent the continuous 5D radiance of a scene, showing impressive performance.
Given a set of posed images of a scene, novel view synthesis produces photo-realistic images at novel viewpoints.
This task is challenging, especially with very sparse input images, since it requires a comprehensive understanding of scenes.
Early work on novel view synthesis utilized image-based rendering~(IBR), which warped input views to target viewpoints and required very dense input views to get high-quality synthesis.
Recently, fast progress has been seen due to the advances in differentiable neural rendering and neural scene representations.
Notably,  neural radiance fields (NeRF~\cite{mildenhall2020nerf})  encodes the continuous 5D radiance of a scene into an MLP and can synthesize impressive results through ray sampling and volumetric rendering. 
However, NeRF requires very dense posed images and extremely slow per-scene optimizations, which is impractical for many applications.


% Despite the impressive synthesis performance, Nerf requires very dense posed images as input and optimization for each scene, which is impractical for many applications.
% Recently, some following works like PixelNerf~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet}, learn scene priors to perform view synthesis from sparse input views without per-scene optimization and achieve impressive performance.
% Nevertheless, these methods still use neural volume rendering like Nerf, which is very extremely slow.


To solve this problem, some recent works like PixelNerf~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet}, 
generalize NeRF by learning a scene prior conditioned on input images and conduct view synthesis in a feed-forward manner. 
They are trained for novel view synthesis with very sparse inputs~(i.e. one or few) and achieve impressive results.
The core of these methods is the backward warping: when sampling a point along the ray, this point is projected to input view planes, and features are extracted based on the projected positions; then these extracted features are taken as inputs for an MLP to predict the RGB and density of the sampled points.
The backward warping obviates the need for input view depth estimations and is expected to achieve high-quality synthesis. 
On the other hand, this backward warping limits the model's efficiency since rendering a single pixel requires hundreds of MLP inferences when sampling points along a ray, which is very slow even without per-scene optimization. 

In this paper,  we revisit this problem and propose that: by combining forward warping and explicit 3D representations, we can achieve comparable performance with existing methods with hundreds of times accelerations for novel view synthesis with very sparse input views. 
Our model explicitly regresses the depth of each input view for a point cloud and employs a high-performance point cloud renderer for novel view synthesis.
With a transformer-based fusion model and view dependence MLP, our method is demonstrated to be able to work efficiently and effectively by experiments. 

Our motivation is also facilitated by the fact that depths can be easily collected using concurrent devices, which intend to be free information in the future. 
Nevertheless, current methods with backward warping and implicit functions gain very little improvement from extra depths since they lack the capacity to use depths directly.
On the contrary, our method can use collected depths naturally and improve the performance with a large margin. 
With the capacity for real-time inference and boosting performance with extra depth inputs, we believe our model would contribute to real-world applications.




==> sections/intro_backup_v2.tex <==
\section{Introduction}
Given several images of a scene, the task of \emph{novel view synthesis} aims to generate photorealistic images depicting the scene from unseen viewpoints.
This long-standing task has significant graphics, virtual, and augmented reality applications, allowing users to explore scenes interactively in 3D.
Recently, Neural Radiance Fields (NeRF)~\cite{mildenhall2020nerf} have emerged as the dominant method for performing novel view synthesis, which uses an MLP to represent 5D radiance fields of scenes \emph{implicitly}.
Despite the impressive results, NeRF is computationally demanding and time-consuming since:
(1) a separate MLP must be learned for each new scene;
(2) generating images requires querying the learned MLP many times for each synthesized pixel.

Some following works as PixelNeRF~\cite{yu2020pixelnerf} and IBRNet~\cite{wang2021ibrnet} have addressed the first of these bottlenecks, 
which are generalizable by modeling neural radiance fields conditioned on a sparse set of input views.
This allows a single model to generate novel views of many unseen scenes without the need for per-scene optimization. 
However, these methods still inherit the same slow image formation process used by NeRF, impeding their practical applications.

A natural question is: \emph{can we achieve a better speed-quality tradeoff ?}
We revisit the image formation process used by NeRF and traditional image-based rendering and propose a fast and generalizable method for NVS with very sparse inputs.
Our method, termed FWD, achieves these goals by replacing \emph{backward warping} with \emph{{\underline F}orward {\underline W}arping}, and eschewing \emph{implicit functions} for \emph{explicit {\underline D}epth}.
It generates images of similar quality to NeRF-like methods~\cite{yu2020pixelnerf,wang2021ibrnet, chen2021mvsnerf} but is orders of magnitude faster.

\input{figures/teaser_figure.tex}
As shown in Figure~\ref{fig:teaser} (I), NeRF-like methods rely on \emph{backward warping}:
for each pixel in the \emph{output} image, they search for its location in the \emph{input} images by casting rays into the scene and projecting them onto the input images.
Since the depth of the output pixel is unknown, many points along the ray must be considered and aggregated.
As shown in Figure~\ref{fig:teaser} (II), much of this computation could be avoided if the depth of the output pixel were known.
In this case, a \emph{single} point in the scene could be projected onto the input views, leading to a dramatic reduction in rendering cost.
Unfortunately, estimating depth for pixels in the \emph{output} view is challenging.
On the other hand, depth in the \emph{input} views is easier to estimate.
If input depth is known, then as shown in Figure~\ref{fig:teaser} (III) we may use \emph{forward warping} to project each pixel in the \emph{input} views onto the \emph{output} views, giving similar computational savings as (II).
% This is the approach we take in this paper.

This idea of \emph{forward warping} is originated in image-based rendering, which typically works by warping, resampling, and/or blending source views to target viewpoints \cite{riegler2020free,choi2019extreme,Riegler2021SVS}.
Despite the impressive speeds, their results are limited by the quality of proxy geometry used for warping.
To get high-quality proxy geometry, very dense input views and/or explicit geometry information are required, hugely restraining the viable scenarios.
In our paper, we show that robust and effective proxy geometry can be learned directly from very sparse input views in an end-to-end manner.


The idea of utilizing explicit depths is also motivated by the increasing prevalence of depth sensors in consumer electronics devices such as the iPhone 12 Pro and the LG G8 ThinQ.
With the growing availability of depth sensors, depths are becoming easy to collect, and we believe it is a significant advantage to use captured depths to improve NVS results further.
We show that if incomplete and noisy depths are available, our proposed method outperforms current methods in both quality and  speed with a large margin, indicating the effectiveness of using  explicit depths.

With explicit depths, our method uses point clouds as the scene representation and warps to target viewpoints through a highly efficient differentiable render. 
To better cope with appearance variance and complicated geometry, we regress the opacity of each point and introduce extra MLP to model the view-dependent effect.
Rather than concentrating point clouds from multi-views, we find using a \emph{per-pixel Transformer}~\cite{46201} to fuse projected pixel features in the output view leads to better performance.
Further, we use a \emph{refinement module} to inpaint projected images and generate the final output.
We validate the effectiveness of our method on ShapeNet, DTU, Common Objects in 3D and a manually collected RGB-D dataset.
We hope that our approach is a step toward building fast, generalizable view synthesis methods that can work in realtime.

\Ang{The current summary is bad. Wait untill finish other parts.}

For summary, our contributions are:
\begin{itemize}
    \item We propose a fast and generalizable novel view synthesis method with very sparse inputs. With forward warping and explicit depths, our method achieves comparable performance while orders of magnitude faster.
    \item With incomplete and noisy depths available, our method outperforms current methods a lot.
    \item We validate our design choices with several ablations.
\end{itemize}



==> sections/intro_backup_v3.tex <==
\section{Introduction}
Given several posed images of a scene, the task of \emph{novel view synthesis}~(NVS) aims to generate photorealistic images depicting the scene from unseen viewpoints.
This long-standing task has significant influence in graphics, VR/AR, allowing users to explore scenes interactively in 3D.
Early work on NVS focuses on \emph{image-based rendering}~(IBR), where models learn to blend a set of reference images for novel views.
In general, light field~\cite{levoy1996light} or proxy geometry~(like mesh surfaces)~\cite{choi2019extreme, hedman2018deep,riegler2020free,Riegler2021SVS} are first constructed from posed input views, and target views are synthesized by resampling or blending source views warped to target viewpoints.
For instance, Hedman et al.~\cite{hedman2018deep} constructed consistent surface meshes by two multi-view stereo algorithms and a CNN was trained to calculate blending weights of a set of ranked image patches (mosaics).
Their performance is fundamentally limited by quality of 3D reconstructions, which requires very dense input views and poses great challenges to geometry estimation algorithms, hugely restraining the viable scenarios.
They are criticized for the artifacts caused by low-quality geometry.
% These methods are fundamentally limited by quality of 3D reconstructions, and generally requires very dense input view and/or explicit geometry, hugely restraining the viable scenarios.

More recently, generalizable NeRF-style methods like PixelNeRF~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet} and MVSNeRF~\cite{chen2021mvsnerf} become more popular and leading methods in this field,
which generate novel views of unseen scenes without  per-scene optimization by modeling neural radiance fields~(NeRF) conditioned on a sparse set of input views.
They query the color and density of every sampling point in the target view from a MLP, and aggregate all points along the ray to get pixel color using \emph{differentiable volumetric rendering}.
With the \emph{backward-warping} style sampling and \emph{differentiable renderer}, these methods eliminate the needs of explicit geometry and learn volume densities optimized for synthesis quality, leading to better quality.
Despite the impressive results, these methods need to query the learned MLP many times for each synthesized pixel, leading to extreme slow speed.

Despite their popularity and preference, we question whether these NeRF-style methods provide optimal speed-quality tradeoff, and revisit the idea of image-based rendering.
We show that with a carefully designed model, comparable performance with tremendous speedup can be achieved by combining \emph{explicit depths} and \emph{differentiable renderer}.
Our method, termed FWD, achieves it with {\underline F}orward {\underline W}arping and explicit {\underline D}epth  estimations.
We construct point clouds from input images by estimating explicit depths  and get novel views via point cloud rendering.
A transformer is utilized to aggregate information from multi-view images.
The whole model  is trained  end-to-end.

Another consideration of utilizing explicit depths is the increasing prevalence of depth sensors in consumer electronics devices such as the iPhone 12 Pro and the LG G8 ThinQ.
With the growing availability of depth sensors, depths are becoming easy to collect, and we believe it is a significant advantage to use captured depths to improve NVS results further.
We show that if incomplete and noisy depths are additionally available, our method outperforms current methods in both quality and  speed with a large margin, indicating the benefits of using  explicit depths.

Our paper focuses on fast and effective novel view synthesis with very sparse inputs, and the scopes of compared methods are specified based on this assumption.
We expect methods to be generalizable and work without per-scene optimization because of efficiency.
Recently numerous NeRF variants have been explored, and some of them also focus on speed, but most of them still require per-scene optimization. 
Fast and generalizable NeRF variants are still an open problem.
We also limit the input views to be sparse, which we believe more useful in practical applications.
This assumption is different from most image-based rendering, and view selection is not available.
Also, sparse input views would pose great challenges to MVS algorithms for getting decent proxy geometry and lead to distinct artifacts.


Our method uses point clouds as the scene representation and renders novel views through a highly efficient differentiable render.
To better cope with appearance variance and complicated geometry, the opacity is regressed for each point, and extra MLP  is introduced to model the view-dependent effect.
Rather than concentrating point clouds from multi-views, we find that using a \emph{per-pixel Transformer}~\cite{46201} to fuse projected pixel features in the output view leads to better performance.
Further, a \emph{refinement module} is employed to inpaint projected images and generate the final output.
We validate the effectiveness of our method on ShapeNet, DTU, Common Objects in 3D and a manually collected RGB-D dataset, and compare with representative NeRF-style and IBR methods. 
We hope that our approach is a step toward building fast, generalizable view synthesis methods that can work in realtime.

\Ang{The current summary is bad. Wait untill finish other parts.}

For summary, our contributions are:
\begin{itemize}
    \item We propose a fast and generalizable novel view synthesis method with very sparse inputs. With forward warping and explicit depths, our method achieves comparable performance while orders of magnitude faster.
    \item With incomplete and noisy depths available, our method outperforms current methods a lot.
    \item We validate our design choices with several ablations.
\end{itemize}



==> sections/intro_backup_v4.tex <==
\section{Introduction}

Given several posed images of a scene, the task of \emph{novel view synthesis}~(NVS) aims to generate photorealistic images depicting the scene from unseen viewpoints.
This long-standing task has applications in graphics, VR/AR, bringing life to still images.
It also requires a deep visual understanding of both geometry and semantics, making it an appealing task to test visual understanding.
\input{figures/teaser_figure.tex}

Early work on NVS focuses on \emph{image-based rendering}~(IBR), where models learn to blend a set of reference images for novel views.
In general, light field~\cite{levoy1996light} or proxy geometry~(like mesh surfaces)~\cite{choi2019extreme, hedman2018deep,riegler2020free,Riegler2021SVS} are first constructed from posed input views, and target views are synthesized by resampling or blending source views warped to target viewpoints.
Their performance is fundamentally limited by the quality of 3D reconstructions, which requires very dense input views and poses significant challenges to geometry estimation algorithms, hugely restraining the viable scenarios.
They are criticized for the \emph{artifacts} caused by low-quality geometry and infeasibility of \emph{sparse inputs},
since it would pose great challenges to MVS algorithms for getting decent proxy geometry and lead to distinct artifacts.

Recently, Neural Radiance Fields (NeRF) ~\cite{mildenhall2020nerf} have become more popular and leading methods for NVS.
They use an MLP to \emph{implicitly} represent the 5D radiance field of the scene,  and query the color and density of every sampling point in the target view from this network.
The color of each pixel is calculated by a volumetric renderer which aggregates colors and densities of all sampling points along the casted ray.
With intensive sampling and \emph{differentiable renderer}, these methods eliminate the need for explicit geometry and learn volume densities optimized for synthesis quality, leading to better quality.
Despite very high-quality results, these methods are not \emph{generalizable}, requiring fitting a separate MLP for each scene with dense view images.
Also, they are extremely \emph{slow} since generating images requires querying the learned MLP tremendous times. 

Some following works emerge as generalizable NeRF variants, like PixelNeRF~\cite{yu2020pixelnerf}, IBRNet~\cite{wang2021ibrnet} and MVSNeRF~\cite{chen2021mvsnerf}, which generate novel views of unseen scenes without per-scene optimization by modeling MLPs conditioned on a sparse set of input views.
However, these generalizable methods still need tremendous times MLP queries for each synthesized pixel, leading to extremely slow speed.
Although some work has explored fast NeRF variants, per-scene optimization is still required.
Fast and generalizable NeRF variants are still an open problem for future work.

In this paper we target a \emph{real-time} and \emph{generalizable} novel view syntheis method with \emph{very sparse inputs}, which is practicle for real-world applications.
Despite their popularity, we question whether these NeRF-style methods provide optimal speed-quality tradeoff and revisit the idea of image-based rendering.
We show that with a carefully designed model, comparable performance with tremendous speedup can be achieved by using \emph{explicit depths} and \emph{differentiable renderer}.
Our method, termed FWD, constructs point clouds from input images and generate novel views by  {\underline F}orward {\underline W}arping features based on estimated {\underline D}epths.

Utilizing explicit depths is also motivated by the increasing prevalence of depth sensors in consumer electronics devices such as the iPhone 12 Pro and the LG G8 ThinQ.
Despite the growing availability of depth sensors and the fact that depths are more accessible to collect than ever, depths are under-explored by  NVS methods. 
We believe it is an appealing advantage if the NVS method can use captured depths to improve NVS quality or speed further.
Although our method could learn to regress depths directly from images, 
it outperforms existing methods in both quality and speed with a large margin if incomplete and noisy sensor depths are additionally available during inference, which indicates the benefits of using explicit depths.

Our method regresses depths for each input view to construct the point cloud and renders novel views via a point cloud renderer. 
Despite the huge accelerations of using explicit depths,  regressing depths from sparse inputs is challenging, limiting the synthesis quality as studied in IBR. 
To address this problem, we employ a differential renderer, which allows the model to construct point cloud optimized for synthesis quality.
A feature vector is regressed for each point for robust representations, and extra MLP is employed to model the view-dependent effect.
Rather than directly concatenating points from different input views, we propose a \emph{per-pixel Transformer}~\cite{46201} to fuse rendered feature maps from arbitrary number input views, resulting in better performance.
Further, a \emph{refinement module} is employed to inpaint fused feature maps and generate the final output.
The whole model is trained end-to-end by photometric loss.

We validate the effectiveness of our method on ShapeNet and DTU benchmark, and compare it with representative NeRF-style and IBR methods. Our method achieves competitive results with SOTA methods while working in realtime,  which is orders of magnitude~(over 140  $\times$) faster.
We hope that our approach is a step toward building fast, generalizable view synthesis methods that can work in realtime.

% \Ang{The current summary is bad. Wait untill finish other parts.}

For summary, our contributions are:
\begin{itemize}[noitemsep,nolistsep]
    \item A fast and generalizable novel view synthesis method with very sparse inputs, which can work in realtime.
    \item An approach to utilize sensor depths when available during inference, leading to significant improvements.
    \item Quantitative and qualitative evaluations on DTU and ShapeNet dataset, showing comparable performance as existing methods with tremendous accelerations.\
    \item Detailed ablation studies for components of design,
\end{itemize}


==> sections/intro_v2.tex <==
\section{Introduction}

% View synthesis task, why it's interesting and important
Given a set of images depicting a scene, the task of \emph{novel view synthesis} aims to generate photorealistic images depicting the scene from unseen viewpoints.
This task has applications in graphics and virtual and augmented reality, since if successful it would bring to life still images, allowing users to interactively explore them in 3D.
View synthesis also requires deep visual understanding of both geometry and semantics, making it an appealing task to test visual understanding.

Recently, Neural Radiance Fields (NeRF)~\cite{mildenhall2020nerf} have emerged as an elegant and effective method for performing view synthesis.
They model scene geometry \emph{implicitly}, and use an MLP to represent 5D radiance fields of scenes.
This approach gives very high-quality results, but it is computationally demanding for two reasons.
First, a separate MLP must be learned for each new scene.
Second, generating image requires querying the learned MLP many times for each synthesized pixel.

The first of these bottlenecks has been addressed by PixelNeRF~\cite{yu2020pixelnerf} and IBRNet~\cite{wang2021ibrnet},
which combine a CNN and MLP to model neural radiance fields conditioned on a sparse set of input views.
This allows a single model to generate novel views of many scenes, and to generalize to new scenes not seen during training.
However these methods inherit the same slow image formation process used by NeRF, so once trained they cannot generate images interactively or in real-time.

Our goal in this paper is to develop a view synthesis method which overcome's both of the aforementioned computational bottlenecks by rethinking the image formation process used by NeRF-like methods.
Our method, termed FWD, achieves these goals by replacing \emph{backward warping} with \emph{{\underline F}orward {\underline W}arping}, and eschewing \emph{implicit functions} for \emph{explicit {\underline D}epth}.
It generates images of similar quality to NeRF-like methods~\cite{yu2020pixelnerf,wang2021ibrnet} but is more than $40\times$ faster.

% \input{figures/teaser_figure.tex}

As shown in Figure~\ref{fig:teaser} (I), NeRF-like methods rely on \emph{backward warping}:
for each pixel in the \emph{output} image, they search for its location in the \emph{input} images by casting rays into the scene and projecting them onto the input images.
Since the depth of the output pixel is unknown, many points along the ray must be considered and aggregated.
As shown in Figure~\ref{fig:teaser} (II), much of this computation could be avoided if the depth of the output pixel were known.
In this case, a \emph{single} point in the scene could be projected onto the input views, leading to a dramatic reduction in rendering cost.
Unfortunately, estimating depth for pixels in the \emph{output} view is challenging.
On the other hand, depth in the \emph{input} views is easier to estimate.
If input depth is known, then as shown in Figure~\ref{fig:teaser} (III) we may use \emph{forward warping} to project each pixel in the \emph{input} views onto the \emph{output} views, giving similar computational savings as (II).
This is the approach we take in this paper.

Our approach requires explicit depth for input views.
Due to the increasing prevalence of depth sensors in consumer electronics devices such as the iPhone 12 Pro and the LG G8 ThinQ, in many cases noisy sensor depth may be available during both training and inference.
If depth is not available at inference, it can be estimated via multiview stereo (MVS) from the sparse input views.
Our experiments demonstrate that our approach is applicable to both settings.
In either case, input depth may be noisy or incomplete;
we thus use a \emph{depth completion module} to refine noisy input depth.

Our approach also requires fusing image information from a set of input views.
To this end we use a \emph{per-pixel Transformer}~\cite{46201} to fuse projected pixel features in the output view.
Our use of forward warping means that some pixels in the output view may be unseen in all input views, leading to holes in the generated image.
We thus use a \emph{refinement module} to fill holes and generate the final output.

Our experiments on the DTU~\cite{jensen2014large} demonstrate that our approach is able to generate images of quality comparable to NeRF-like methods~\cite{yu2020pixelnerf,wang2021ibrnet} but is more than $40\times$ faster.
Though our method assumes access to noisy input depth during inference, we believe that this assumption is not unrealistic due to the growing availability of depth sensors, and is also a small price to pay for the massive speedups we achieve compared to prior methods.
We hope that our approach is a step toward building fast, generalizable view synthesis methods that can work in realtime.



==> sections/method_backup_v5.tex <==
\section{Method}

Given a sparse set of input images $\{I_{i}\}_{i=1}^{N}$ and corresponding camera poses $\{R_i, T_i\}$,
our goal is to synthesize a novel view with camera pose $\{R_t, T_t\}$ fast and effectively.
The depths $\{D^{sen}_{i}\}$ of $I_i$ captured from sensors are optionally available, which are generally incomplete and noisy.
% The incomplete and noisy depths of each input image $\{D^{sen}_{i}\}$ are optionally available, which are obtained from depth sensor. 

The insight of our method is that using explicit depths and forward warping enables real-time rendering speed and tremendous accelerations. 
Meanwhile, to alleviate quality degradations caused by inaccurate depth estimations,  a differentiable renderer and well-designed fusion \& refinement modules are required, encouraging the model to learn geometry and features optimized for synthesis quality.

As illustrated in Figure \ref{fig:model}, with estimated depths, input view~$I_{i}$ is converted to a 3D point cloud~$\mathcal{P}_{i}$ containing geometry and view-dependent semantics of the view.  
A differentiable neural point cloud renderer $\pi$ is used to project point clouds to target viewpoints. 
Rather than directly aggregating point clouds across views before rendering, we propose a Transformer-based module $T$ fusing rendered results at target view. 
Finally, a refinement module $R$ is employed to generate final outputs.
The whole model is trained end-to-end with photometric and perceptual loss. 
% We describe point cloud construction in Sec. \ref{sec:met_pce}, point cloud renderer in Sec. \ref{sec:met_p}, and target view fusion and refinement in Sec. \ref{sec:met_fr}.

\subsection{Point Cloud Construction}\label{sec:met_pce}
% The point cloud $\mathcal{P}_i$ at input view $I_{i}$ is constructed by estimating $\{ D_i, F'_i \}$ using three networks: Spatial Feature  Encoder $f$,  Depth Network $d$ and View-Dependent Feature MLP $W$.
% $f$ encodes per-pixel feature vectors $F_i$ and $d$ estimates depths $D_i$ at the same resolution as the input image.
% $F_i$ is concatenated with location-specific information and passed through $W$ yielding view-dependent features $F'_i$.
Using an explicit 3D representation is a natural way to inject 3D priors into the model.
% For realistic synthesis, a 3D representation is expected, injecting 3D priors and rules into the model. 
We use point clouds to represent scenes due to their efficiency, compact memory usage, and scalability to complex scenes.
For input view $I_i$, we construct point cloud $\mathcal{P}_{i}$ by estimating per-pixel depth $D_i$ and per-pixel feature vectors $F'_i$ at the same resolution as the input image, then projecting the feature vectors into 3D space using known camera intrinsics.
The depth $D_i$ is estimated by a \emph{depth network} $d$, giving 3D scene structure;
features $F'_i$ are computed by a \emph{spatial feature encoder} $f$ and \emph{view-dependent MLP} $\psi$, representing scene semantics.
\par \noindent {\bf Spatial Feature Encoder $f$.}
Scene semantics of input view $I_i$ are mapped to pixel-specific feature vectors $F_i$ by spatial feature encoder $f$.
Each feature vector in $F_i$ is 61-dimensions and is concatenated with RGB channels for 64 dimensions.
$f$ is built on BigGAN architecture~\cite{brock2018large}.
 
\par \noindent {\bf Depth Network $d$.}
% Our method estimates depths for each input view via depth network $d$.
Estimating depth from a single image has scaling/shifting ambiguity, losing valuable multi-view cues and leading to inconsistent estimations across views.
Applying multi-view stereo algorithms~(MVS)~\cite{schoenberger2016mvs,yao2018mvsnet,wang2020patchmatchnet} solely on sparse inputs is challenging because of limited overlap and huge baselines between input views, leading to inaccurate and low-confidence estimations.
Therefore, we employ a hybrid design cascading a U-Net after the MVS module.
The U-Net takes image $I_i$ and estimated depths from the MVS module as inputs, refining depths with multi-view stereo cues and image cues. 
PatchmatchNet~\cite{wang2020patchmatchnet} is utilized as the MVS module, which is fast and lightweight.
% U-Net and PatchmatchNet are learnable.

\par \noindent {\bf Depth Estimation with sensor depths.}
As stated, U-Net receives an initial depth estimation from the MVS module and outputs a refined depth used to build the point cloud.   
If sensor depth $D^{sen}_{i}$ is available,  it is directly input to the U-Net as the initial depth estimations. 
In this setting, U-Net servers as completion and refinement module taking $D^{sen}_{i}$ and $I_i$ as inputs, since  $D^{sen}_{i}$ is usually noisy and incomplete.
During training,  loss $L_{s}$ is employed to encourage the U-Net output to match the sensor depth.
\begin{align}
    \mathcal{L}_{s} = \| M_i \odot D_i - M_i \odot D^{sen}_{i} \|
\end{align}
where $M_i$ is a binary mask indicating valid sensor depths.


\par \noindent {\bf View-Dependent Feature MLP $\psi$.}
The appearance of the same object varies across views because of lighting and view direction changes, introducing inconsistency between multiple views.
The scene semantics is represented by spatial features $F_i$ and translated to the target view for synthesis. 
Therefore, view direction changes from input to target views should be inserted into scene semantics to model the view-dependent effects. 
We design an MLP $\psi$ to compute view-dependent spatial features $F'_i$ by taking $F_i$ and relative view changes $\Delta v$ as inputs.
For each point in the cloud, $\Delta v$ is calculated based on normalized view directions $v_i$ and $v_t$,  from the point to camera centers of input view $i$ and target view $t$.
The relative view direction change is calculated as: 
\begin{align}
	\Delta v = [(v_i - v_t) / \| v_i - v_t \|, v_i \cdot v_t], v_i, v_t \in \mathbb{R}^3.
\end{align}
and the view-dependent feature $F'_i$  is:
\begin{align}
	F'_{i} = \psi(F_{i}, \delta(\Delta v))
\end{align}
where $\delta$ is a two-layer MLP mapping $\Delta v$ to a 32-dimensions vector and $\psi$ is also a two-layer MLP.


\subsection{Point Cloud Renderer}\label{sec:met_p}
After constructing a point cloud $\mathcal{P}_i$ from view $i$ containing the geometry and semantics of the scene, we expect to view $\mathcal{P}_i$ at target views for synthesis. 
We use a neural point cloud $\pi$ to achieve it.
$\mathcal{P}_i$ is first transformed to target view coordinates based on relative camera poses and then rendered by $\pi$.
The rendered results $\tilde{F}_i$ are spatial feature maps, sharing the same dimension as feature $F'_i$ in $\mathcal{P}_{i}$ at each pixel.
With explicit geometry transformation and renderer satisfying geometry rules, our rendered results are geometrically consistent and correct across views.

As discussed, we expect this renderer to be \emph{differentiable} for quality. 
To achieve it, the renderer splats points to the image plane and gets pixel values by blending features of points intersected with this pixel.
The blending weights are computed based on depths and distance to pixels. The render is implemented using Pytorch3D~\cite{ravi2020accelerating}.
% \begin{align}
%     \omega_i = \frac{o_i \cdot \exp(o_i \cdot r_i \cdot \frac{\tilde{d_i}}{\gamma})}{\exp(\frac{\epsilon}{\gamma}) + \sum_{k}o_k \cdot r_i \cdot \exp(o_k \cdot \frac{\tilde{d_k}}{\gamma})}
% \end{align}
% where $o_i$ is the opacity, $\tilde{d_i}$ is the normalized depth ranging from 0 to 1, $r_i = \min(1, \frac{\| \vec{r_i}\|_2}{R_i})$, $\vec{r_i}$ is the orthogonal vector pointing from the center of point $i$ to ray and $R_i$ is the predefined radius.  
% $\gamma$ controls the softness of blending.

This fully differentiable renderer allows our model to be trained end-to-end, where photometric and perceptual loss gradients can be propagated to points' position and features.   
In this way, the model learns to estimate depths and features optimized for synthesis quality, leading to superior quality.
We show the effectiveness of it in experiments.
\subsection{Fusion and Refinement}\label{sec:met_fr}

We fuse the point clouds constructed from each input view for synthesis. 
A naive fusion translates each point cloud to target view coordinates and aggregates them into a large one for rendering. 
Despite high efficiency, it is vulnerable to inaccurate depths since points with wrong depths may occlude points from other views, leading to degraded performance.
Some regularizers like PointNet may be feasible to apply on the aggregated point cloud for refinement, but they are not efficient when point number is large.

Therefore,  we instead render each point cloud individually at the target viewpoint and fuse the rendered results.
We propose a novel Transformer-based fusion module $T$ to fuse arbitrary size inputs and use a refinement module $R$ to synthesize final results based on fused features.

\input{figures/model_figure2.tex}
\par \noindent {\bf Fusion Transformer $T$.}
Given a set of feature maps $\{\tilde{F}_i\}$ rendered from point clouds,
we fuse them into one feature map, which will be decoded into an RGB image by refinement module. 
The fusion operation should understand scene semantics, be fast and support arbitrary number of inputs in any order. 
We take advantage of progress on the Transformer and propose a pixel-wise Transformer $T$ for fusion, which is detailed in Figure~\ref{fig:model2}.
$T$ extracts feature vectors from $\{\tilde{F}_i\}$ as inputs and output fused one at each pixel.
It applies standard multi-head attention to the sequence of feature vectors and queries using an extra learnable ``token".
Applied on features, $T$ utilizes scene semantics for fusion.


Fusing rendered feature maps may lose some helpful geometry information since it projects 3D to 2D.
For instance, point clouds from different views may have meaningful occlusion relationships based on their relative depths. 
Also, rendered feature maps from views closer to target views are more robust and important than ones from distant views.
To this end, we render depths at target view for each point cloud and compute the relative view changes from input to target views.
We concatenate them as geometry features and use them as position encoding of the Transformer.  

\par \noindent {\bf Refinement Module $R$.}
Refinement module $R$ decodes fused feature maps $\tilde{F}$ to RGB images $\tilde{I}$ at target view. 
It will inpaint regions not visible in the input views in a semantically meaningful and geometrically accurate manner.
Also, it corrects local errors caused by inaccurate depths and improves perceptual quality based on semantics contained by feature maps, leading to coherent and high-quality synthesis. 
$R$ is built with 8 ResNet~\cite{he2016deep} blocks.

% We do not use an adversarial loss, finding it prevents the model from learning accurate depths.

% \input{figures/model_figure2.tex}

\subsection{Training and Implementation Details}
\label{sec:method_details}
Our model is trained end-to-end with photometric $\mathcal{L}_{l_2}$ and perceptual $\mathcal{L}_{c}$ losses between generated and ground-truth target images.
% When sensor depths are available during inference, loss $\mathcal{L}_{s}$  is employed.
% Adding sensor depths as an extra supervision only for training is also explored in our experiments,
The whole loss function is:
\begin{align}
	\mathcal{L} = \lambda_{l_2}\mathcal{L}_{l_2} + \lambda_{c} \mathcal{L}_c 
\end{align}

where $\lambda_{l_2}=5.0, \lambda_{c}=1.0$.
% \lambda_{s}=5.0$.
The model is trained end-to-end on 4 2080Ti GPUs for 2 days, using Adam~\cite{kingma2014adam} with learning rate $10^{-4}$ and $\beta_1{=}0.9, \beta_2{=}0.999$.
When sensors depths are available as inputs, $\mathcal{L}_{s}$  is used with $\lambda_{s}=5.0$.
% Each mini-batch includes 16 scenes, where each scene contains 3 input views and 1 target view.





==> sections/method_copy_v4.tex <==
\input{figures/model_figure.tex}

\section{Method}

Given a sparse set of input images $\{I_{i}\}_{i=1}^{N}$ and corresponding camera poses $\{R_i, T_i\}$,
our goal is to synthesize a novel view with camera pose $\{R_t, T_t\}$ fast and effectively.
The depths $\{D^{sen}_{i}\}$ captured by sensors are optionally available, which are generally incomplete and noisy.
% The incomplete and noisy depths of each input image $\{D^{sen}_{i}\}$ are optionally available, which are obtained from depth sensor. 

The insight of our method is that using explicit depths and forward warping enables real-time rendering speed and tremendous accelerations. 
Meanwhile, to alleviate quality degradations caused by inaccurate depth estimations,  a differentiable renderer, and a well-designed fusion \& refinement module are required, encouraging the model to learn geometry and features optimized for synthesis quality.

As illustrated in Figure \ref{fig:model}, we use a point cloud representation and high-performance point cloud renderer, which requires only a single forward pass for view synthesis.
Separate point clouds $\mathcal{P}_i$ are computed for each input view, enabling the model to learn view-dependent features without a radiance field.
Rather than directly aggregating point clouds from each view and rendering target view images, we generate target views by fusing rendered results from each input view with a Transformer $T$ and applying refinement module $R$ for final results. 
The whole model is trained end-to-end with photometric loss and perceptual loss.
We describe point cloud construction in Sec. \ref{sec:met_pce}, point cloud renderer in Sec. \ref{sec:met_p}, and target view fusion and refinement in Sec. \ref{sec:met_fr}.

\subsection{Point Cloud Construction}\label{sec:met_pce}
The point cloud $\mathcal{P}_i$ at input view $I_{i}$ is constructed by estimating $\{ D_i, F'_i \}$ using three networks: Spatial Feature  Encoder $f$,  Depth Network $d$ and View-Dependent Feature MLP $W$.
$f$ encodes per-pixel feature vectors $F_i$ and $d$ estimates depths $D_i$ at the same resolution as the input image.
$F_i$ is concatenated with location-specific information and passed through $W$ yielding view-dependent features $F'_i$.

\par \noindent {\bf Spatial Feature Encoder $f$.}
$f$ takes image $I_{i}$ and outputs pixel-specific feature vectors $F_i$, which encode high-level representations such as scene semantics.
Each feature vector in $F_i$ is 61-dimensions and is concatenated with 3 input RGB channels, for a total of 64 dimensions.
Following prior work \cite{wiles2020synsin}, $f$ is built on BigGAN architecture\cite{brock2018large}.

\par \noindent {\bf Depth Network $d$.}
Although regressing depths independently for each view like SynSin~\cite{wiles2020synsin} gives reasonable relative depths, it suffers from depth scaling/shifting ambiguity and inconsistency between multi-view depths.
Applying multi-view stereo algorithms~(MVS)~\cite{schoenberger2016mvs,yao2018mvsnet,wang2020patchmatchnet} on sparse input images is challenging because of limited overlaps and huge baselines between input views, leading to inaccurate estimations and regions with low confidence.
Therefore, we employ a U-Net as a depth refinement module, taking image $I_i$  and MVS estimated depths as inputs.
It refines depths considering cues from MVS and images.
PatchmatchNet~\cite{wang2020patchmatchnet} is utilized as the MVS module, which is fast and lightweight.
U-Net and PatchmatchNet are learnable.

\par \noindent {\bf Depth Estimation with sensor depths.}
If depth sensors like structured-light scanner or LiDAR are available, sensor depths $D^{sen}_{i}$ can be easily captured, which are usually with noise and missing regions.
In this setting, depth network $d$ serves as a depth completion and refinement module, which estimates the refined depth $D_i$ given $I_i$ and $D^{sen}_{i}$.
MVS estimated depths are not needed since sensor depths already provide enough geometry information. 
$\mathcal{L}_{s}$ is employed to encourage depth network to utilize sensor depths. 
\begin{align}
    \mathcal{L}_{s} = \| M_i \odot D_i - M_i \odot D^{sen}_{i} \|
\end{align}
where $M_i$ is a binary mask indicating valid sensor depths.


\par \noindent {\bf View-Dependent Feature MLP $W$.}
The appearance of objects varies between different views, and points may have various colors across views because of lighting. 
To model this phenomenon, we design an MLP $W$ to compute view-dependent spatial features $F'_i$ by taking spatial features $F_i$  and relative view changes $\Delta v_i$ as inputs.
Similar to \cite{wang2021ibrnet}, for each point, $\Delta v_i$ is calculated based on normalized view direction vector $v_i$ and  $v_t$, which direct from the point to camera centers of input view $i$ and target view $t$.
The relative view changes $\Delta v$ is a 4-dims vector, where the first three dims are normalized view direction differences, and the last dim is the inner product of view direction vectors.
\begin{align}
	\Delta v = [(v_i - v_t) / \| v_i - v_t \|, v_i \cdot v_t], v_i, v_t \in \mathbb{R}^3.
\end{align}
and the view dependent feature $F'_i$ for point $x$ is:
\begin{align}
	F'_{i} = W(F_{i}, \delta(\Delta v))
\end{align}
where $\delta$ is a two-layer MLP mapping $\Delta v$ to a 32-dims vector and $W$ is also a two-layer MLP.


\subsection{Point Cloud Renderer}\label{sec:met_p}
Given a constructed point cloud $\mathcal{P}_i$ from view $i$,
we project it to the target view by a point cloud renderer $\pi$.
$\mathcal{P}_i$ is first geometrically translated into target view coordinate according to relative camera poses and then rendered by $\pi$.
Since $\mathcal{P}_{i}$ employs vectors $F'_{i}$ rather than RGB values as its features, the rendered results $\tilde{F}_i$ are spatial feature maps as well, sharing the same vector length as $F'_i$ at each pixel.

As discussed, we expect this renderer to be \emph{fast} and \emph{differentiable} for speed and quality. 
We use the highly-efficient renderer in Pytorch3D~\cite{ravi2020accelerating}, which splats points to a region and accumulates them based on blending weights for each pixel.
The weight is computed based on depth, distance to rays cast from the pixel, and sphere radius.
% \begin{align}
%     \omega_i = \frac{o_i \cdot \exp(o_i \cdot r_i \cdot \frac{\tilde{d_i}}{\gamma})}{\exp(\frac{\epsilon}{\gamma}) + \sum_{k}o_k \cdot r_i \cdot \exp(o_k \cdot \frac{\tilde{d_k}}{\gamma})}
% \end{align}
% where $o_i$ is the opacity, $\tilde{d_i}$ is the normalized depth ranging from 0 to 1, $r_i = \min(1, \frac{\| \vec{r_i}\|_2}{R_i})$, $\vec{r_i}$ is the orthogonal vector pointing from the center of point $i$ to ray and $R_i$ is the predefined radius.  
% $\gamma$ controls the softness of blending.

This fully differentiable renderer allows our model to be trained end-to-end, where photometric and perceptual loss gradients can be computed w.r.t points' position and features.   
In this way, the model learns to estimate depths and features optimized for synthesis quality, leading to superior quality.
We show the effectiveness of it in experiments.
\subsection{Fusion and Refinement}\label{sec:met_fr}

Given a set of point clouds constructed from each input view, fusion is required to synthesize novel views.
A naive fusion can be achieved by translating each point cloud to target view coordinates and aggregating them into a large point cloud for rendering. 
Despite its high efficiency, it is vulnerable to inaccurate depth estimations since points with inaccurate depths from one input view may occlude or pollute points from other views, leading to degraded performance.
Some regularizers like PointNet may be feasible to apply on the aggregated point cloud for refinement, but they are not efficient when point number is large.


Based on the above considerations,  we would instead render feature maps at target view for each point cloud individually and fuse feature maps.
To deal with an arbitrary number of input views, we use a Transformer $T$ to aggregate features from different input views.

\input{figures/model_figure2.tex}
\par \noindent {\bf Fusion Transformer $T$.}
We propose a pixel-wise Transformer $T$ fusing feature vectors from $N$ input views for every position in the target view, which is detailed in Figure~\ref{fig:model2}.
We collect a set of feature vectors $\tilde{f}_i$ from rendered feature maps $\tilde{F}_i$ at a certain position as the inputs of Transformer and take the output as the vector of fused feature maps at the same location.
Our Transformer applies standard multi-head attention to the sequence of feature vectors and queries the fused features using an extra learnable "token".
Although fusion is conducted pixel-wise, the input features contain high-level semantic information and are expected to give abundant semantic cues for fusion.

Fusing rendered feature maps may lose some helpful geometry information since it projects 3D space to 2D.
For instance, point clouds from different views may have meaningful occlusion relationships based on their relative depths. 
Also, rendered feature maps from views closer to target views are more robust and important than feature maps from distant views.
To this end, we also render the depths at target view for each point cloud and compute the relative view changes from 
We concatenate them as geometry features and use them as position encoding of the Transformer.  

\par \noindent {\bf Refinement Module $R$.}
Even if the features are projected accurately, regions not visible in the input views will be empty in the target views.
To this end, we utilize a refinement module $R$ to inpaint missing regions in a semantically meaningful and geometrically accurate manner.
$R$ takes fused features $\tilde{F}$ as input and outputs target view images $\tilde{I}$.
Following ~\cite{wiles2020synsin}, $R$ consists of 8 ResNet \cite{he2016deep} blocks with Batch Normalization injected with noise \cite{brock2018large}.
% We do not use an adversarial loss, finding it prevents the model from learning accurate depths.

% \input{figures/model_figure2.tex}

\subsection{Training and Implementation Details}
\label{sec:method_details}
Our model is trained end-to-end with photometric $\mathcal{L}_{l_2}$ and perceptual $\mathcal{L}_{c}$ losses between generated and ground-truth target images.
% When sensor depths are available during inference, loss $\mathcal{L}_{s}$  is employed.
% Adding sensor depths as an extra supervision only for training is also explored in our experiments,
The whole loss function is:
\begin{align}
	\mathcal{L} = \lambda_{l_2}\|I_{GT} - \tilde{I}\|^2 + \lambda_{c} \mathcal{L}_c 
\end{align}

where $\lambda_{l_2}=5.0, \lambda_{c}=1.0$.
% \lambda_{s}=5.0$.
The model is trained end-to-end on 4 2080Ti GPUs for 2 days, using Adam~\cite{kingma2014adam} with learning rate $10^{-4}$ and $\beta_1{=}0.9, \beta_2{=}0.999$.
When sensors depths are available as inputs, $\mathcal{L}_{s}$  is used with $\lambda_{s}=5.0$.
% Each mini-batch includes 16 scenes, where each scene contains 3 input views and 1 target view.





==> sections/related_work_backup.tex <==
\section{Related Work}
Novel view synthesis is a long-standing problem in computer vision, which allows for the generation of new views of a scene given one or more images. 
Recent progress has been driven by learned scene representations. 
These representations are either explicit and implicit and vary in approach along with number of views and information available at inference.

\par \noindent {\bf Geometric Scene Representations.} 
Classical methods often use depth maps ~\cite{penner2017soft, chaurasia2013depth} or multi-view geometry \cite{chen1993view, debevec1996modeling, 1640800, zitnick2004high, penner2017soft}, while learned geometry can produce good performance given less input images and information \cite{choi2019extreme, tulsiani2018layer}.
Advances in differentiable rendering \cite{liu2019soft, jiang2020sdfdiff, chen2019learning} have allowed these methods to learn 3D end-to-end without explicit supervision.
These methods learn a variety of 3D representations, including depth and multi-plane images \cite{tatarchenko2016multi, zhou2018stereo, srinivasan2019pushing, penner2017soft, chaurasia2013depth}, voxels \cite{sitzmann2019deepvoxels}, meshes \cite{riegler2020free, hedman2018instant, hu2020worldsheet}, and point clouds \cite{wiles2020synsin, liu2020infinite}.
In this work, we use a point cloud representation.

Learned geometric representations rely heavily on rendering and refinement \cite{yu2018generative, yang2017high, brock2018large, wang2018high} to inpaint missing information and improve realism in novel viewpoints.
Refinement has improved dramatically owing to advances in generative modeling \cite{ledig2017photo, karras2020analyzing, zhang2019self, CycleGAN2017}, while rendering frameworks \cite{ravi2020accelerating, jatavallabhula2019kaolin, najibi2020dops, huang2020lstm} have also facilitated progress.
Yet, information across viewpoints is typically aggregated before rendering \note{cite}, making it difficult to condition views on one another.
We propose to render viewpoints separately and combine using transformer attention \cite{46201, dosovitskiy2020image, carion2020end}. 

Recent work learns a 3D representation to synthesize views given only a single image \cite{wiles2020synsin, hu2020worldsheet, single_view_mpi, liu2020infinite}.
Not only does this require minimal information, it is highly efficient, since a single representation can be repeatedly rendered across viewpoints.
Nevertheless, learning a robust scene representation with few views and no 3D supervision is challenging, so strong supervision such as depth can be used \cite{shih20203d, song2015sun, silberman2012indoor, tulsiani2018factoring, hedman2016scalable}.
This is facilitated by the growing availability of annotated depth maps \cite{dai2017scannet, Matterport3D, NIPS2016_0deb1c54, aanaes2016large}.
We find using annotated depth with a geometric representation yields the efficiency of an explicit representation with highly competitive performance given only a few images.


If multiple images available, 3D information can be inferred for view synthesis.
Traditional methods generate photometrical images by utilizing depth maps ~\cite{penner2017soft, chaurasia2013depth}, multi-view geometry \cite{debevec1998efficient, debevec1996modeling, fitzgibbon2005image, kopf2013image, seitz2006comparison, zitnick2004high}
or 4D functions~\cite{levoy1996light,gortler1996lumigraph}.
In the deep learning era, learning based methods show impressive performance with various 3D representations, 
including depth images \cite{aliev2020, meshry2019neural, riegler2020free, yoon2020novel},
multi-plane images \cite{single_view_mpi, zhou2018stereo},
point clouds \cite{wiles2020synsin}, voxels \cite{liu2020neural, sitzmann2019deepvoxels}, meshes \cite{hu2020worldsheet, kato2018neural, liu2019soft}, multi-layer meshes \cite{hedman2018instant, shih20203d}, and radiance fields \cite{mildenhall2020nerf, zhang2020nerf++}.

\subsection{Neural Scene Representation}
Our work is closely related to the recent progress of neural scene representation~\cite{genova2020local,jiang2020local,mescheder2019occupancy,park2019deepsdf,niemeyer2020differentiable,saito2019pifu,sitzmann2019deepvoxels},
which uses neural networks to represent the shape and appearance of scenes. 
For instance, NeRF \cite{mildenhall2020nerf,zhang2020nerf++} represents the scene by encoding a 5D neural radiance field to a MLP network. 
Despite the impressive performance, NeRF must be optimized for each new scene, taking a long time to converge.
More recently works~\cite{wang2021ibrnet, yu2020pixelnerf, trevithick2020grf}try to address this issue by learning a shared prior and generalizing NeRF without per-scene optimization, with a focus on very sparse input views.
However, these work still suffers from the very slow speed of volumetric rendering of the NeRF. 
To this end, we propose to use point cloud for high-speed rendering with the same focus on very few input views. 

\subsection{Differentiable Point Cloud Renderer}
We utilize a highly-efficient differentiable neural point cloud renderer for end-to-end training of the model.
Differentiable renderer ~\cite{jiang2020sdfdiff,niemeyer2020differentiable,liu2020dist, liu2019soft} is a recent hot-spot problem among deep learning and graphics, 
and differentiable point cloud neural renderer~\cite{wiles2020synsin,lassner2020pulsar,aliev2020}gets more attention considering it is efficient in both time and memory usage.
In our paper, we employ the point cloud renderer proposed by ~\cite{wiles2020synsin}.


==> sections/related_work_v2.tex <==
\section{Related Work}
Novel view synthesis is a long-standing problem in computer vision, which allows for the generation of new views of a scene given one or more images. 
Recent progress has been driven by learned scene representations. 
These representations are either explicit and implicit and vary in approach along with number of views and information available at inference.

\par \noindent {\bf Geometric Scene Representations.} 
Classical methods often use depth maps ~\cite{penner2017soft, chaurasia2013depth} or multi-view geometry \cite{chen1993view, debevec1996modeling, zitnick2004high, penner2017soft}, while learned geometry can produce good performance given less input images and information \cite{choi2019extreme, tulsiani2018layer}.
Advances in differentiable rendering \cite{liu2019soft, jiang2020sdfdiff, chen2019learning,niemeyer2020differentiable,liu2020dist} have allowed these methods to learn 3D end-to-end without explicit supervision.
These methods learn a variety of 3D representations, including depth and multi-plane images \cite{tatarchenko2016multi, zhou2018stereo, srinivasan2019pushing, penner2017soft, chaurasia2013depth}, voxels \cite{sitzmann2019deepvoxels}, meshes \cite{riegler2020free, hedman2018instant, hu2020worldsheet}, and point clouds \cite{wiles2020synsin, liu2020infinite}.
In this work, we use a point cloud representation, which enables us to use efficient point cloud rendering \cite{wiles2020synsin,lassner2020pulsar,aliev2020}

Learned geometric representations rely heavily on rendering and refinement \cite{yu2018generative, yang2017high, brock2018large, wang2018high} to inpaint missing information and improve realism in novel viewpoints.
Refinement has improved dramatically owing to advances in generative modeling \cite{ledig2017photo, karras2020analyzing, zhang2019self, CycleGAN2017}, while rendering frameworks \cite{ravi2020accelerating, jatavallabhula2019kaolin, najibi2020dops, huang2020lstm} have also facilitated progress.
Although information across viewpoints is typically aggregated before rendering~\cite{lombardi2019neural}, 
% making it difficult to condition views on one another.
we propose to render viewpoints separately and combine using a transformer \cite{46201, dosovitskiy2020image, carion2020end}, which enables attention across input views.

% Recent work learns a 3D representation to synthesize views given only a single image \cite{wiles2020synsin, hu2020worldsheet, single_view_mpi, liu2020infinite}.
% Not only does this require minimal information, it is highly efficient, since a single representation can be repeatedly rendered across viewpoints.
% Nevertheless, learning a robust scene representation with few views and no 3D supervision is challenging, so strong supervision such as depth can be used \cite{shih20203d, song2015sun, silberman2012indoor, tulsiani2018factoring, hedman2016scalable}.
% This is facilitated by the growing availability of annotated depth maps \cite{dai2017scannet, Matterport3D, NIPS2016_0deb1c54, aanaes2016large}.
% We find using annotated depth with a geometric representation yields the efficiency of an explicit representation with highly competitive performance given only a few images.
Recent work learns a 3D representation to synthesize views given only a single image \cite{wiles2020synsin, hu2020worldsheet, single_view_mpi, liu2020infinite}.
Despite the impressive results, these methods are limited to small view changes and struggle beyond a margin. 
Our methods take few views as input expecting distinct view changes.
Also, learning a robust scene representation with few views and no 3D supervision is challenging, so strong supervision such as depth can be used \cite{shih20203d, song2015sun, silberman2012indoor, tulsiani2018factoring, hedman2016scalable}.
This is facilitated by the growing availability of annotated depth maps \cite{dai2017scannet, Matterport3D, NIPS2016_0deb1c54, aanaes2016large}. Additionally, progress in learned depth proxies such as multi-view stereo \cite{wang2020patchmatchnet, luo2020consistent, Huang2018, yao2018mvsnet} enable use of depth at test time without ground truth.
We find using annotated depth with a geometric representation yields the efficiency of an explicit representation with highly competitive performance given only a few images. We show this is true using true depth or learned MVS depth.

\par \noindent {\bf Neural Scene Representations.} 
Recent work also learns implicit scene representations for view synthesis \cite{rombach2021geometry, liu2020neural, genova2020local, jiang2020local, mescheder2019occupancy, park2019deepsdf}.
Given many views, neural radiance fields~(NeRF) have shown impressive capacity to model viewpoint-specific appearance \cite{mildenhall2020nerf, zhang2020nerf++, martinbrualla2020nerfw, park2020nerfies, wang2021nerf},
though require expensive per-scene optimization.
Recent methods~\cite{wang2021ibrnet, yu2020pixelnerf, trevithick2020grf,chen2021mvsnerf, jain2021putting} address this issue by learning a shared prior and generalizing NeRF without per-scene optimization, with a focus on very sparse input views.
Nevertheless, these methods require expensive ray sampling are therefore slow at inference.
% In contrast, our method requires no optimization and uses a geometric representation which can be rendered repeatedly for fast inference.
In contrast, our method achieves tremendous accelerations using a geometric representation.

To accelerate NeRF, some concurrent work proposes to reformulate the computation pipeline~\cite{garbin2021fastnerf}, precompute and store it as novel representations~\cite{yu2021plenoctrees,hedman2021baking},
and even explore adding view dependence to explicit 3D representations~\cite{liu2020neural,wizadwongsa2021nex}.
However, these methods still rely on per-scene optimization and dense input views, while our method requires no optimization during inference.
% To accelerate NeRF, some concurrent work combine

% \note{What about the fast nerf rendering stuff (fastnerf, plenoctrees, baking nerf)? that is concurrent; and does it not work for few views?}


==> tables/depth_ablation.tex <==
\begin{table*}[t]
    \centering
    \caption{
    \textbf{Ablation study using different depths.}
    We investigate different strategy for depth learning.
    GT Depth utilize the captured depths as extra input.
    MVS Depth estimates the depths from input images via MVS algorithms.
    UNet Depth regresses depth directly for each input image.
    Supervised Depth follows the same architecture as UNet Depth, while depths are trained supervised during training.}
    \vspace{-1in}

    \begin{tabular}{p{3cm} p{2.5cm} p{2cm} p{2.5cm} p{2.5cm}}
    \toprule[2pt]
    model & PSNR & SSIM & LPIPS & Inference Time\\
    \midrule
    GT Depth &21.08 & 0.748& 0.181 &1.203s \\
    MVS Depth &17.55 & 0.621 & 0.302 &1.364s \\
    UNet Depth& 16.36 & 0.532& 0.347 &1.200s\\
    Supervised Depth &16.61 &0.547 &0.334 &1.200s\\
    \bottomrule [2 pt]
    \end{tabular}

    \label{tab:depth_ablation}
\end{table*}

==> tables/dtu.tex <==
\begin{table*}[t!]
\caption{{\bf Quantitative comparison on DTU real images}. 
Results using PSNR, and SSIM, and LPIPS. Our image quality is similar to NeRF-based methods without depth supervision, while being significantly faster.
While NeRF-based models are not suited to use depth, an explicit scene representation can easily train using depth to boost performance.
%Results using Perc Sim \cite{zhang2018unreasonable} and L1 distance. 
%To discourage predicting mean pixels, 
%we compute percentage within x\% for some x: the amount of predictions within an arbitrary distance of ground truth.
%The autoregressive model is more likely to be highly similar to the ground truth, while completions may differ substantially.
%In contrast, the base model is more likely to predict mean pixels to minimze average distance to ground truth.
}
%\setlength{\tabcolsep}{5pt} 
\centering 
\resizebox{\ifdim\width>\linewidth%\columnwidth
        \linewidth%\columnwidth
      \else
        \width
      \fi}{!}
{
  \begin{tabular}{l l c c c c c c c c c c c c c c c c}
    \toprule
 & & Scene No. & 8 & 21 & 30 & 31 & 34 & 38 & 40 & 41 & 45 & 55 & 63 & 82 & 103 & 110 & 114 \\
     & & Average & Apple & Buildings & Pumpkin & Food & Bricks & Wood & Temple & Pail & Bodywash & Rabbit & Fruit & Elf & Pig & Gold & Buddha \\
% & 8 & 21 & 30 & 31 & 34 & 38 & 40 & 41 & 45 & 55 & 63 & 82 & 103 & 110 & 114\\
\midrule
\multirow{4}{*}{PSNR $\uparrow$} & IBRNet \cite{wang2021ibrnet} & 18.86 &18.86 & 15.05 & 21.17 & 16.68 & 17.41 & 14.83 & 17.14& 18.84 & 15.72 & 24.38 & 21.43 & 18.98 & 18.34& 21.44 & 22.68  \\
& PixelNeRF \cite{yu2020pixelnerf} & 18.99 & 19.22 & 15.52 & 22.43 & 17.78 & 17.23 & 15.97 & 18.40 & 18.85 & 15.37 & 20.68 & 21.22 & 20.57 & 19.82 & 20.11 &19.68  \\
& FWD (MVS) & 17.55 & 18.36 & 14.26 & 15.79 & 15.44 & 18.61 & 16.33 & 16.29 & 16.74 & 16.78 & 20.29 & 17.51 & 15.27 & 18.85 & 21.15 & 21.60 \\
& FWD (GT) & \textbf{21.08} & 20.36 & 16.95 & 23.68 & 17.64 & 22.73 & 18.48 & 20.35 & 21.30 & 18.46 & 24.07 & 23.24 & 20.86 & 22.59 & 21.81 &23.71 \\
\midrule
\multirow{4}{*}{SSIM $\uparrow$} & IBRNet \cite{wang2021ibrnet} & 0.695  & 0.745 & 0.464 & 0.855 & 0.628 & 0.597 & 0.471 & 0.615 & 0.704 & 0.643 & 0.743 & 0.863 & 0.821 & 0.714 & 0.775 &788  \\
& PixelNeRF \cite{yu2020pixelnerf} & 0.680 & 0.763 & 0.477 &0.959 &0.677 & 0.540 & 0.511 & 0.636 & 0.681 & 0.608 & 0.670 & 0.829 & 0.794 & 0.686 & 0.773 & 0.671  \\
& FWD (MVS) & 0.621 & 0.706 & 0.393 & 0.739 & 0.559 & 0.601 & 0.496 & 0.547 & 0.588 & 0.592 & 0.630 & 0.752 & 0.688 & 0.653 & 0.658 &0.721 \\
& FWD (GT) & \textbf{0.748} & 0.768 & 0.622 & 0.868 & 0.693 & 0.730 & 0.660 & 0.715 & 0.737 & 0.713 & 0.726 & 0.872 & 0.843 & 0.781 & 0.704 &0.794 \\
\midrule
\multirow{4}{*}{LPIPS $\downarrow$} & IBRNet \cite{wang2021ibrnet} & 0.387 & 0.377 & 0.510 & 0.252 & 0.431 & 0.466 & 0.533 & 0.430 & 0.389 & 0.393 & 0.395 & 0.219 & 0.264 & 0.414 & 0.377 & 0.357 \\
& PixelNeRF \cite{yu2020pixelnerf} & 0.399 &0.362 & 0.520 & 0.211 & 0.394 & 0.496 & 0.532 & 0.435 & 0.453 & 0.437 & 0.433 & 0.230 & 0.253 & 0.428 & 0.389 & 0.406  \\
& FWD (MVS) & 0.302 & 0.283 & 0.374 & 0.284 & 0.305 & 0.320 & 0.359 & 0.350 & 0.338 & 0.252 & 0.311 & 0.238 & 0.290 & 0.327 & 0.264 &0.237 \\
& FWD (GT) & \textbf{0.181} & 0.187 & 0.220 & 0.111 & 0.190 & 0.195 & 0.236 & 0.198 & 0.184 & 0.156 & 0.202 & O.120 & 0.138 & 0.212 & 0.206 & 0.170 \\

  \bottomrule
\end{tabular}
\vspace{-1in}
}
\label{tab:dtu}
\end{table*}


==> tables/method_depth_table.tex <==
%\begin{table*}[h]
    %\centering
    %\caption{
    %\textbf{Settings for different methods.}
    %We summary settings including the availability of GT depths during training and inference, depth network input for baseline and ablated models.  }
\begin{wraptable}{r}{0.35\textwidth}
    \centering
    \vspace{-3mm}
    \scalebox{0.825}{
    \begin{tabular}{p{2.05cm} P{0.4cm} P{0.4cm} P{1.3cm}}
    \toprule%[2pt]
& \multicolumn{2}{c}{Use depth} & Depth \\
    Model & Train & Test & Details \\
\midrule
    FWD (GT) & \checkmark & \checkmark & Incomplete \\
    FWD (MVS) & \checkmark &  & Noisy \\
    FWD (Sup.) & \checkmark & & - \\
    FWD (Unsup.) & & & - \\
 IBRNet \cite{wang2021ibrnet} & & & - \\
PixelNeRF \cite{yu2020pixelnerf} & & & - \\
    \bottomrule% [2 pt]
    \end{tabular}}
    \label{tab:method_settings_table}
    \vspace{-1mm}
    \caption{
      Use of depth data for different versions of our method
      and baselines.
    }
    \label{tab:method_settings_table}
    \vspace{-2mm}
\end{wraptable}


==> tables/multi_inputs.tex <==
\begin{table*}[ht!]
    \centering
    \caption{We investigate the novel view synthesis performance and speed when provided with more input views. }
    \resizebox{\ifdim\width>\linewidth%\columnwidth
        \linewidth%\columnwidth
      \else
        \width
      \fi}{!}
    {
    \begin{tabular}{ l |c c c c | c c c c| c c c c}
    \toprule[2pt]
      &\multicolumn{4}{c}{3 views} &\multicolumn{4}{c}{6 views} &\multicolumn{4}{c}{9 views} \\
      &PSNR & SSIM &LPIPS & Time &PSNR & SSIM &LPIPS & Time &PSNR & SSIM &LPIPS & Time\\
    \midrule
    PixelNeRF &18.99 &0.680 &0.399 &30min &19.96 &0.712 &0.372 & 54min &20.47 &0.734 &0.348 & 72 min\\
    IBRNet &18.86 & 0.695 & 0.387 & 173s & 20.93 & 0.780 & 0.312 & 245s & 21.30 & 0.805 & 0.285 & 319s \\
    FWD (MVS) &17.55 &0.621 &0.302 &1.364s &18.83 &0.680 &0.258 & 4.82&18.98 & 0.691 &0.247 &7.75  \\
    FWD (GT) &21.08 & 0.748 &0.182 &1.203s & 21.32 &0.755 &0.177 & 1.604s &21.53 &0.764 &0.168 & 2.214s\\

    
    \bottomrule [2 pt]
    
    \end{tabular}
    }
    \label{tab:multiview}
\end{table*}


==> tables/time_analyse.tex <==
\begin{table}[t]
    \centering
    \caption{
    \textbf{ Inference time.}
    We evaluate times used for each process in one forward pass with a batch size of 24. }
    \resizebox{0.48\textwidth}{!}{
        \centering
        \begin{tabular}{p{1.3cm} p{1cm} p{1cm} p{1cm} p{1cm} p{1.2cm} p{1cm}}
        \toprule[2pt]
         & Constr. & Render & Fusion &Refine. & Total\\
         \midrule
        Time~(ms) &40.39 &172.57 & 70.11 & 302.59 &585.66 \\
        Percent  & 6.90 & 29.47 & 11.97 & 61.67 & 100.00\\
        \bottomrule [2 pt]
        \end{tabular}}
    \label{tab:time}
\end{table}



==> tables/time_table.tex <==
\begin{table*}[t]
    \centering
    \caption{
    \textbf{ Inference time.}
    We evaluate  the per-scene inference time and corresponding FPS of our model with different resolutions, including 46 target views.
    % We report the inference time with and without view-dependent feature for each model.
    Our method can achieve orders-of-magnitude accelerations accelerations compared existing methods.  }
    \resizebox{\ifdim\width>\linewidth%\columnwidth
        \linewidth%\columnwidth
      \else
        \width
      \fi}{!}
{
    \begin{tabular}{ m{2cm}  m{2.5 cm} m{2.5cm} m{2.5 cm} m{2.5cm} m{2.5 cm}}
    \toprule[2pt]
       & Low Resolution & Hybrid  & Full Resolution & PixelNeRF & IBRNet\\
       \midrule
    FWD (MVS) &  1.24s/37.1FPS &1.37s/33.6FPS & 4.50s/ 10.2FPS&  \multirow{2}{*}{30min/0.025FPS}&  \multirow{2}{1.5cm}{173s/0.265FPS}\\

    FWD (GT )  & 1.04s/45.1FPS &1.20s/38.3FPS   & 3.70s/12.4FPS \\

    \bottomrule [2 pt]
    \end{tabular}
}
    \label{tab:time}
\end{table*}

==> tables/time_table_v2.tex <==
\begin{wraptable}{r}{0.4\textwidth}
  \centering
  \scalebox{0.8}{
  \begin{tabular}{rccc}
    \toprule
    Method & Resolution & Time & FPS \\
    \midrule
    \multirow{3}{*}{FWD (GT)} & $150\times200$ & 1.24s & 37.1 \\
    & Hybrid & 1.37s & 33.6 \\
    & $300\times400$ & 4.5s & 10.2 \\
    \midrule
    \multirow{3}{*}{FWD (MVS)} & $150\times200$ & 1.04s & 45.1 \\
    & Hybrid & 1.20s & 38.3 \\
    & $300\times400$ & 3.7s & 12.4 \\
    \midrule
    PixelNeRF~\cite{yu2020pixelnerf} & $300\times400$ & 30m & 0.03 \\
    IBRNet~\cite{wang2021ibrnet} & $300\times400$ & 173s & 0.27 \\
    \bottomrule
  \end{tabular}}
  \caption{
    Speed comparision for inference-time forward passes at different resolutions.
    We measure the total time to synthesize 46 target views for a scene; FPS amortizes shared computation for all output views.
  }
  \vspace{-5mm}
  \label{tab:time}
\end{wraptable}


==> tables/user_study.tex <==
\begin{table}[t]
    \centering
    \caption{
    \textbf{User study.}
    We conduct A/B test for DTU synthesis results, asking users to pick results with better quality.
    We show the preference frequency of method A~(row methods) over method B~(column method).
    Our methods are consistently preferred.}
    \resizebox{0.48 \textwidth}{!}{
        \begin{tabular}{p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{1.5cm}}
    \toprule[2pt]
    A / B & \FWD & \FWDds & \FWDrgbd &PixelNeRF &IBRNet\\
    \midrule
    \FWD &- &21.5\% &1.5\%  &65.6\% &77.8\% \\
    \FWDds &-  &-  &8.9\%  &96.9\%  &93.9\% \\
    \FWDrgbd &-  &-  &- &99.6\%  & 97.5\%  \\
    \bottomrule [2 pt]
    \end{tabular}}
    \label{tab:user_study}
    \vspace{-5mm}
\end{table}
